An axiomatic approach to analytic $1$-affineness

The notion of $1$-affineness was originally formulated by Gaitsgory in the context of derived algebraic geometry. Motivated by applications to rigid and analytic geometry, we introduce two very general and abstract frameworks where it makes sense to ask for objects to be $1$-affine with respect to some sheaf of categories. The first framework is suited for studying the problem of $1$-affineness when the sheaf of categories arises from an operation in a six-functor formalism over $\mathscr{C}$; we apply it to the setting of analytic stacks and condensed mathematics. The second one concerns $1$-affineness in the context of quasi-coherent sheaves of categorical modules over stable module categories: it simultaneously generalizes the algebro-geometric setting of Gaitsgory and makes it possible to formulate the problem also when dealing with rigid analytic varieties and categories of nuclear modules.

==> Bibliography.tex <==
@misc{ramzi2024locallyrigidinftycategories,
      title={Locally rigid $\infty$-categories}, 
      author={Maxime Ramzi},
      year={2024},
      eprint={2410.21524},
      archivePrefix={arXiv},
      primaryClass={math.CT},
      url={https://arxiv.org/abs/2410.21524}, 
}

% @book{huber2013etale,
%   title={{\'E}tale cohomology of rigid analytic varieties and adic spaces},
%   author={Huber, Roland},
%   volume={30},
%   year={2013},
%   publisher={Springer}
% }

% @book{bosch2014lectures,
%   title={Lectures on formal and rigid geometry},
%   author={Bosch, Siegfried},
%   volume={2105},
%   year={2014},
%   publisher={Springer}
% }

@misc{ramzi2024dualizablepresentableinftycategories,
      title={Dualizable presentable $\infty$-categories}, 
      author={Maxime Ramzi},
      year={2024},
      eprint={2410.21537},
      archivePrefix={arXiv},
      primaryClass={math.CT},
      url={https://arxiv.org/abs/2410.21537}, 
}

@misc{anschutz2024,
      title={Descent for solid quasi-coherent sheaves on perfectoid spaces}, 
      author={Johannes Anschütz and Lucas Mann},
      year={2024},
      eprint={2403.01951},
      archivePrefix={arXiv},
      primaryClass={math.AG},
      url={https://arxiv.org/abs/2403.01951}, 
}

@article{Bambozzi_2018,
   title={Stein domains in Banach algebraic geometry},
   volume={274},
   ISSN={0022-1236},
   url={http://dx.doi.org/10.1016/j.jfa.2018.01.003},
   DOI={10.1016/j.jfa.2018.01.003},
   number={7},
   journal={Journal of Functional Analysis},
   publisher={Elsevier BV},
   author={Bambozzi, Federico and Ben-Bassat, Oren and Kremnizer, Kobi},
   year={2018},
   month=apr, pages={1865–1927} }

@misc{benbassat2024perspectivefoundationsderivedanalytic,
      title={A Perspective on the Foundations of Derived Analytic Geometry}, 
      author={Oren Ben-Bassat and Jack Kelly and Kobi Kremnizer},
      year={2024},
      eprint={2405.07936},
      archivePrefix={arXiv},
      primaryClass={math.AG},
      url={https://arxiv.org/abs/2405.07936}, 
}

@misc{kelly2025localisinginvariantsderivedbornological,
      title={Localising invariants in derived bornological geometry}, 
      author={Jack Kelly and Devarshi Mukherjee},
      year={2025},
      eprint={2505.15750},
      archivePrefix={arXiv},
      primaryClass={math.KT},
      url={https://arxiv.org/abs/2505.15750}, 
}

@misc{efimov2025localizinginvariantsinverselimits,
      title={Localizing invariants of inverse limits}, 
      author={Alexander I. Efimov},
      year={2025},
      eprint={2502.04123},
      archivePrefix={arXiv},
      primaryClass={math.KT},
      url={https://arxiv.org/abs/2502.04123}, 
}

@misc{efimov2025ktheorylocalizinginvariantslarge,
      title={K-theory and localizing invariants of large categories}, 
      author={Alexander I. Efimov},
      year={2025},
      eprint={2405.12169},
      archivePrefix={arXiv},
      primaryClass={math.KT},
      url={https://arxiv.org/abs/2405.12169}, 
}

@misc{raksit2020hochschildhomologyderivedrham,
      title={Hochschild homology and the derived de Rham complex revisited}, 
      author={Arpon Raksit},
      year={2020},
      eprint={2007.02576},
      archivePrefix={arXiv},
      primaryClass={math.AG},
      url={https://arxiv.org/abs/2007.02576}, 
}

@article{Ben_Zvi_2018,
   title={Integrating quantum groups over surfaces},
   volume={11},
   ISSN={1753-8424},
   url={http://dx.doi.org/10.1112/topo.12072},
   DOI={10.1112/topo.12072},
   number={4},
   journal={Journal of Topology},
   publisher={Wiley},
   author={Ben‐Zvi, David and Brochier, Adrien and Jordan, David},
   year={2018},
   month=aug, pages={874–917} }

@misc{haine2022,
      title={Descent for sheaves on compact Hausdorff spaces}, 
      author={Peter J. Haine},
      year={2022},
      eprint={2210.00186},
      archivePrefix={arXiv},
      primaryClass={math.AT},
      url={https://arxiv.org/abs/2210.00186}, 
}

@misc{geometrizationreallanglands,
  title={Geometrization of the real local Langlands correspondence},
  author={Scholze, Peter},
  year={2024},
  url={https://people.mpim-bonn.mpg.de/scholze/RealLocalLanglands.pdf},
}

@misc{kunneth6ff,
      title={Categorical K\"unneth formulas for analytic stacks}, 
      author={Youshua Kesting},
      year={2025},
      eprint={2507.08566},
      archivePrefix={arXiv},
      primaryClass={math.AG},
      url={https://arxiv.org/abs/2507.08566}, 
}

@misc{GLC5,
      title={Proof of the geometric Langlands conjecture V: the multiplicity one theorem}, 
      author={Dennis Gaitsgory and Sam Raskin},
      year={2024},
      eprint={2409.09856},
      archivePrefix={arXiv},
      primaryClass={math.AG},
      url={https://arxiv.org/abs/2409.09856}, 
}

@misc{GLC4,
      title={Proof of the geometric Langlands conjecture IV: ambidexterity}, 
      author={D. Arinkin and D. Beraldo and L. Chen and J. Faergeman and D. Gaitsgory and K. Lin and S. Raskin and N. Rozenblyum},
      year={2024},
      eprint={2409.08670},
      archivePrefix={arXiv},
      primaryClass={math.AG},
      url={https://arxiv.org/abs/2409.08670}, 
}

@misc{GLC3,
      title={Proof of the geometric Langlands conjecture III: compatibility with parabolic induction}, 
      author={Justin Campbell and Lin Chen and Joakim Faergeman and Dennis Gaitsgory and Kevin Lin and Sam Raskin and Nick Rozenblyum},
      year={2024},
      eprint={2409.07051},
      archivePrefix={arXiv},
      primaryClass={math.AG},
      url={https://arxiv.org/abs/2409.07051}, 
}

@misc{GLC2,
      title={Proof of the geometric Langlands conjecture II: Kac-Moody localization and the FLE}, 
      author={D. Arinkin and D. Beraldo and J. Campbell and L. Chen and J. Faergeman and D. Gaitsgory and K. Lin and S. Raskin and N. Rozenblyum},
      year={2024},
      eprint={2405.03648},
      archivePrefix={arXiv},
      primaryClass={math.AG},
      url={https://arxiv.org/abs/2405.03648}, 
}

@misc{GLC1,
      title={Proof of the geometric Langlands conjecture I: construction of the functor}, 
      author={Dennis Gaitsgory and Sam Raskin},
      year={2024},
      eprint={2405.03599},
      archivePrefix={arXiv},
      primaryClass={math.AG},
      url={https://arxiv.org/abs/2405.03599}, 
}

@misc{stefanich2023tan,
      title={Tannaka duality and 1-affineness}, 
      author={Germán Stefanich},
      year={2023},
      eprint={2311.04515},
      archivePrefix={arXiv},
      primaryClass={math.AG},
      url={https://arxiv.org/abs/2311.04515}, 
}

@misc{mair2021,
      title={Animated Condensed Sets and Their Homotopy Groups}, 
      author={Catrin Mair},
      year={2021},
      eprint={2105.07888},
      archivePrefix={arXiv},
      primaryClass={math.AT},
      url={https://arxiv.org/abs/2105.07888}, 
}

@misc{heyer6ff2024,
      title={6-Functor Formalisms and Smooth Representations}, 
      author={Claudius Heyer and Lucas Mann},
      year={2024},
      eprint={2410.13038},
      archivePrefix={arXiv},
      primaryClass={math.CT},
      url={https://arxiv.org/abs/2410.13038}, 
}

@misc{kelly2025,
      title={Localising invariants in derived bornological geometry}, 
      author={Jack Kelly and Devarshi Mukherjee},
      year={2025},
      eprint={2505.15750},
      archivePrefix={arXiv},
      primaryClass={math.KT},
      url={https://arxiv.org/abs/2505.15750}, 
}

@book{bosch1984non,
  title={Non-archimedean analysis},
  author={Bosch, Siegfried and G{\"u}ntzer, Ulrich and Remmert, Reinhold},
  volume={261},
  year={1984},
  publisher={Springer Berlin}
}

@phdthesis{fedeli2023topological,
  title={Topological Hochschild homology of adic rings},
  author={Fedeli, Adriano C{\'o}rdova},
  year={2023},
  school={PhD thesis, University of Copenhagen}
}

@misc{camargo2024analytic,
      title={The analytic de Rham stack in rigid geometry}, 
      author={Juan Esteban Rodríguez Camargo},
      year={2024},
      eprint={2401.07738},
      archivePrefix={arXiv},
      primaryClass={math.AG},
      url={https://arxiv.org/abs/2401.07738}, 
}

@book{toen2008homotopical,
  title={Homotopical Algebraic Geometry II: Geometric Stacks and Applications: Geometric Stacks and Applications},
  author={To{\"e}n, Bertrand and Vezzosi, Gabriele},
  volume={2},
  year={2008},
  publisher={American Mathematical Soc.}
}

@misc{clausenlectures,
  title={Condensed Mathematics and Complex Geometry},
  author={Clausen, Dustin and Scholze, Peter},
  year={2022},
  url={https://people.mpim-bonn.mpg.de/scholze/Complex.pdf},
}

@misc{analytic,
  title={Lectures on Analytic Geometry},
  author={Clausen, Dustin and Scholze, Peter},
  year={2020},
  url={https://www.math.uni-bonn.de/people/scholze/Analytic.pdf},
}

@misc{six-functors-scholze,
title={Six functor formalisms},
author={Scholze, Peter},
year={2023},
url={https://people.mpim-bonn.mpg.de/scholze/SixFunctors.pdf},
}

@misc{CamargoDerivedRigid,
  author = {Camargo, Juan Esteban Rodr{\'\i}guez},
  title = {Six functor formalism for solid quasi-coherent sheaves on rigid spaces},
  YEAR = {2024},
  url = {https://bogdanzavyalov.com/refs/seminars/analytic-k-theory/L8.pdf},
}


@book {huber2013etale,
    AUTHOR = {Huber, Roland},
     TITLE = {\'Etale cohomology of rigid analytic varieties and adic
              spaces},
    SERIES = {Aspects of Mathematics},
    VOLUME = {E30},
 PUBLISHER = {Friedr. Vieweg \& Sohn, Braunschweig},
      YEAR = {1996},
     PAGES = {x+450},
      ISBN = {3-528-06794-2},
   MRCLASS = {14G22 (14F20)},
  MRNUMBER = {1734903},
MRREVIEWER = {Lorenzo\ Ramero},
       DOI = {10.1007/978-3-663-09991-8},
       URL = {https://doi.org/10.1007/978-3-663-09991-8},
}

@article{porta2016higher,
  title={Higher analytic stacks and GAGA theorems},
  author={Porta, Mauro and Yu, Tony Yue},
  journal={Advances in Mathematics},
  volume={302},
  pages={351--409},
  year={2016},
  publisher={Elsevier}
}

@article{porta2018derived,
  title={Derived non-archimedean analytic spaces},
  author={Porta, Mauro and Yu, Tony Yue},
  journal={Selecta Mathematica},
  volume={24},
  pages={609--665},
  year={2018},
  publisher={Springer}
}

@misc{soor2024sixfunctorformalismquasicoherentsheaves,
      title={A six-functor formalism for quasi-coherent sheaves and crystals on rigid-analytic varieties}, 
      author={Arun Soor},
      year={2024},
      eprint={2409.07592},
      archivePrefix={arXiv},
      primaryClass={math.NT},
      url={https://arxiv.org/abs/2409.07592}, 
}

@misc{meyer2024derived,
      title={Derived $q$-Hodge complexes and refined $\operatorname{TC}^-$}, 
      author={Samuel Meyer and Ferdinand Wagner},
      year={2024},
      eprint={2410.23115},
      archivePrefix={arXiv},
      primaryClass={math.AT},
      url={https://arxiv.org/abs/2410.23115}, 
}

% @misc{kesting2025categoricalkunnethformulasanalytic,
%       title={Categorical K\"unneth formulas for analytic stacks}, 
%       author={Youshua Kesting},
%       year={2025},
%       eprint={2507.08566},
%       archivePrefix={arXiv},
%       primaryClass={math.AG},
%       url={https://arxiv.org/abs/2507.08566}, 
% }

@misc{liu2024enhancedoperationsbasechange,
      title={Enhanced six operations and base change theorem for higher Artin stacks}, 
      author={Yifeng Liu and Weizhe Zheng},
      year={2024},
      eprint={1211.5948},
      archivePrefix={arXiv},
      primaryClass={math.AG},
      url={https://arxiv.org/abs/1211.5948}, 
}

@book {mann2022p,
    AUTHOR = {Mann, Lucas},
     TITLE = {A p-{A}dic 6-{F}unctor {F}ormalism in {R}igid-{A}nalytic
              {G}eometry},
      NOTE = {Thesis (Ph.D.)--Rheinische Friedrich-Wilhelms-Universitaet
              Bonn (Germany)},
 PUBLISHER = {ProQuest LLC, Ann Arbor, MI},
      YEAR = {2022},
     PAGES = {290},
      ISBN = {9798304998956},
   MRCLASS = {99-05},
  MRNUMBER = {4890351},
       URL =
              {https://gateway.proquest.com/openurl?url_ver=Z39.88-2004&rft_val_fmt=info:ofi/fmt:kev:mtx:dissertation&res_dat=xri:pqm&rft_dat=xri:pqdiss:31909601},
}

@misc{mikami2023fppf,
      title={Fppf-descent for condensed animated rings}, 
      author={Yutaro Mikami},
      year={2023},
      eprint={2311.13408},
      archivePrefix={arXiv},
      primaryClass={math.AG},
      url={https://arxiv.org/abs/2311.13408}, 
}

@misc{andreychev2023ktheorieadischerraume,
      title={$K$-Theorie adischer R\"aume}, 
      author={Grigory Andreychev},
      year={2023},
      eprint={2311.04394},
      archivePrefix={arXiv},
      primaryClass={math.KT},
      url={https://arxiv.org/abs/2311.04394}, 
}

@article{mathew2016galois,
    AUTHOR = {Mathew, Akhil},
     TITLE = {The {G}alois group of a stable homotopy theory},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {291},
      YEAR = {2016},
     PAGES = {403--541},
      ISSN = {0001-8708,1090-2082},
   MRCLASS = {14F35 (11F11 11S20 14F20 18D10 18G55 55P43 55U35)},
  MRNUMBER = {3459022},
MRREVIEWER = {Rui\ Miguel\ Saramago},
       DOI = {10.1016/j.aim.2015.12.017},
       URL = {https://doi.org/10.1016/j.aim.2015.12.017},
}

@misc{andreychev2021pseudocoherent,
      title={Pseudocoherent and Perfect Complexes and Vector Bundles on Analytic Adic Spaces}, 
      author={Grigory Andreychev},
      year={2021},
      eprint={2105.12591},
      archivePrefix={arXiv},
      primaryClass={math.AG},
      url={https://arxiv.org/abs/2105.12591}, 
}

@misc{bosco2023p,
      title={On the $p$-adic pro-\'etale cohomology of Drinfeld symmetric spaces}, 
      author={Guido Bosco},
      year={2023},
      eprint={2110.10683},
      archivePrefix={arXiv},
      primaryClass={math.NT},
      url={https://arxiv.org/abs/2110.10683}, 
}

@misc{clausen2019lectures,
  title={Lectures on condensed mathematics},
  author={Clausen, Dustin and Scholze, Peter},
  url={https://www.math.uni-bonn.de/people/scholze/Condensed.pdf},
  year={2019}}


@article {jacinto2022solidlocallyanalyticrepresentations,
    AUTHOR = {Rodrigues Jacinto, Joaqu\'in and Rodr\'iguez Camargo, Juan
              Esteban},
     TITLE = {Solid locally analytic representations of {$p$}-adic {L}ie
              groups},
   JOURNAL = {Represent. Theory},
  FJOURNAL = {Representation Theory. An Electronic Journal of the American
              Mathematical Society},
    VOLUME = {26},
      YEAR = {2022},
     PAGES = {962--1024},
      ISSN = {1088-4165},
   MRCLASS = {11F85 (22E41 22E50)},
  MRNUMBER = {4475468},
MRREVIEWER = {Anton\ Deitmar},
       DOI = {10.1090/ert/615},
       URL = {https://doi.org/10.1090/ert/615},
}

@misc{preygel2011thomsebastianidualitymatrix,
      title={Thom-Sebastiani and Duality for Matrix Factorizations}, 
      author={Anatoly Preygel},
      year={2011},
      eprint={1101.5834},
      archivePrefix={arXiv},
      primaryClass={math.AG},
      url={https://arxiv.org/abs/1101.5834}, 
}

@article {neeman_grothendieck_duality,
    AUTHOR = {Neeman, Amnon},
     TITLE = {The {G}rothendieck duality theorem via {B}ousfield's
              techniques and {B}rown representability},
   JOURNAL = {J. Amer. Math. Soc.},
  FJOURNAL = {Journal of the American Mathematical Society},
    VOLUME = {9},
      YEAR = {1996},
    NUMBER = {1},
     PAGES = {205--236},
      ISSN = {0894-0347,1088-6834},
   MRCLASS = {18E30 (14F05)},
  MRNUMBER = {1308405},
MRREVIEWER = {Luca\ Barbieri Viale},
       DOI = {10.1090/S0894-0347-96-00174-9},
       URL = {https://doi.org/10.1090/S0894-0347-96-00174-9},
}

@article {serre2,
    AUTHOR = {Serre, Jean-Pierre},
     TITLE = {Un th\'eor\`eme de dualit\'e},
   JOURNAL = {Comment. Math. Helv.},
  FJOURNAL = {Commentarii Mathematici Helvetici},
    VOLUME = {29},
      YEAR = {1955},
     PAGES = {9--26},
      ISSN = {0010-2571,1420-8946},
   MRCLASS = {56.0X},
  MRNUMBER = {67489},
MRREVIEWER = {S.\ Chern},
       DOI = {10.1007/BF02564268},
       URL = {https://doi.org/10.1007/BF02564268},
}


@article {braden2016conical,
    AUTHOR = {Braden, Tom and Licata, Anthony and Proudfoot, Nicholas and
              Webster, Ben},
     TITLE = {Quantizations of conical symplectic resolutions {II}: category
              {$\mathcal{O}$} and symplectic duality},
      NOTE = {with an appendix by I. Losev},
   JOURNAL = {Ast\'erisque},
  FJOURNAL = {Ast\'erisque},
    NUMBER = {384},
      YEAR = {2016},
     PAGES = {75--179},
      ISSN = {0303-1179,2492-5926},
      ISBN = {978-2-85629-845-9},
   MRCLASS = {53D50 (14F05 14J81 16S38 17B10)},
  MRNUMBER = {3594665},
}






@article {MR2430869,
    AUTHOR = {Lu, Di Ming and Palmieri, John H. and Wu, Quan Shui and Zhang,
              James J.},
     TITLE = {Koszul equivalences in {$A_\infty$}-algebras},
   JOURNAL = {New York J. Math.},
  FJOURNAL = {New York Journal of Mathematics},
    VOLUME = {14},
      YEAR = {2008},
     PAGES = {325--378},
      ISSN = {1076-9803},
   MRCLASS = {16E45 (16E35 16S37)},
  MRNUMBER = {2430869},
MRREVIEWER = {Mikael\ Vejdemo Johansson},
       URL = {http://nyjm.albany.edu:8000/j/2008/14_325.html},
}






@book {sabbah,
    AUTHOR = {Sabbah, Claude},
     TITLE = {Isomonodromic deformations and {F}robenius manifolds},
    SERIES = {Universitext},
   EDITION = {French},
      NOTE = {An introduction},
 PUBLISHER = {Springer-Verlag London, Ltd., London; EDP Sciences, Les Ulis},
      YEAR = {2007},
     PAGES = {xiv+279},
      ISBN = {978-1-84800-053-7; 978-2-7598-0047-6},
   MRCLASS = {32G34 (32S30 32S40 33E50 34M45 53D45)},
  MRNUMBER = {2368364},
}


	@misc{pavia1,
	doi = {10.48550/ARXIV.2207.11994},
	url = {https://arxiv.org/abs/2207.11994},
	author = {Pavia, Emanuele},
	keywords = {Category Theory (math.CT), Algebraic Geometry (math.AG), K-Theory and Homology (math.KT), FOS: Mathematics, FOS: Mathematics},
	title = {A $t$-structure on the $\infty$-category of mixed graded modules},
	publisher = {arXiv},
	year = {2022},
	copyright = {arXiv.org perpetual, non-exclusive license}
}


@article{pavia2,
title = {Mixed graded structure on Chevalley-Eilenberg functors},
journal = {Advances in Mathematics},
volume = {448},
pages = {109721},
year = {2024},
issn = {0001-8708},
doi = {https://doi.org/10.1016/j.aim.2024.109721},
url = {https://www.sciencedirect.com/science/article/pii/S0001870824002366},
author = {Emanuele Pavia},
}


@article {compositionproduct,
	AUTHOR = {Haugseng, Rune},
	TITLE = {{$\infty$}-operads via symmetric sequences},
	JOURNAL = {Math. Z.},
	FJOURNAL = {Mathematische Zeitschrift},
	VOLUME = {301},
	YEAR = {2022},
	NUMBER = {1},
	PAGES = {115--171},
	ISSN = {0025-5874},
	MRCLASS = {18N70},
	MRNUMBER = {4405646},
	DOI = {10.1007/s00209-021-02881-w},
	URL = {https://doi-org.pros1.lib.unimi.it/10.1007/s00209-021-02881-w},
}


@article {geometryoffiltrations,
	AUTHOR = {Moulinos, Tasos},
	TITLE = {The geometry of filtrations},
	JOURNAL = {Bull. Lond. Math. Soc.},
	FJOURNAL = {Bulletin of the London Mathematical Society},
	VOLUME = {53},
	YEAR = {2021},
	NUMBER = {5},
	PAGES = {1486--1499},
	ISSN = {0024-6093},
	MRCLASS = {14F08 (14A20 55P42)},
	MRNUMBER = {4335221},
	DOI = {10.1112/blms.12512},
	URL = {https://doi-org.pros1.lib.unimi.it/10.1112/blms.12512},
}


@article {fubini,
	AUTHOR = {Chach\'{o}lski, Wojciech and Scherer, J\'{e}r\^{o}me},
	TITLE = {Homotopy theory of diagrams},
	JOURNAL = {Mem. Amer. Math. Soc.},
	FJOURNAL = {Memoirs of the American Mathematical Society},
	VOLUME = {155},
	YEAR = {2002},
	NUMBER = {736},
	PAGES = {x+90},
	ISSN = {0065-9266},
	MRCLASS = {55P65 (18G55 55U30)},
	MRNUMBER = {1879153},
	MRREVIEWER = {Timothy Porter},
	DOI = {10.1090/memo/0736},
	URL = {https://doi.org/10.1090/memo/0736},
}


@book {tannakaduality,
	AUTHOR = {Schauenburg, Peter},
	TITLE = {Tannaka duality for arbitrary {H}opf algebras},
	SERIES = {Algebra Berichte [Algebra Reports]},
	VOLUME = {66},
	PUBLISHER = {Verlag Reinhard Fischer, Munich},
	YEAR = {1992},
	PAGES = {ii+57},
	ISBN = {3-88927-100-6},
	MRCLASS = {18D10 (16W30 18F99)},
	MRNUMBER = {1623637},
}


@misc{bialgebrasmonoidalstructure,
	doi = {10.48550/ARXIV.1810.00734},
	url = {https://arxiv.org/abs/1810.00734},
	author = {Beardsley, Jonathan},
	keywords = {Algebraic Topology (math.AT), FOS: Mathematics, FOS: Mathematics, 55N22, 55P43, 16T10, 18N70, 18F20},
	title = {On Bialgebras, Comodules, Descent Data and Thom Spectra in $\infty$-categories},
	publisher = {arXiv},
	year = {2018},	
	copyright = {arXiv.org perpetual, non-exclusive license}
}


@misc{yonedaisnatural1,
	doi = {10.48550/ARXIV.2011.11042},
	
	url = {https://arxiv.org/abs/2011.11042},
	
	author = {Haugseng, Rune and Hebestreit, Fabian and Linskens, Sil and Nuiten, Joost},
	
	keywords = {Category Theory (math.CT), Algebraic Topology (math.AT), FOS: Mathematics, FOS: Mathematics, 18N60, 18N70},
	
	title = {Two-variable fibrations, factorisation systems and $\infty$-categories of spans},
	
	publisher = {arXiv},
	
	year = {2020},
	
	copyright = {Creative Commons Attribution Non Commercial No Derivatives 4.0 International}
}


@misc{yonedaisnatural2,
	doi = {10.48550/ARXIV.2209.12575},
	
	url = {https://arxiv.org/abs/2209.12575},
	
	author = {Ramzi, Maxime},
	
	keywords = {Category Theory (math.CT), FOS: Mathematics, FOS: Mathematics},
	
	title = {The Yoneda embedding is natural},
	
	publisher = {arXiv},
	
	year = {2022},
	
	copyright = {arXiv.org perpetual, non-exclusive license}
}


@misc{yonedaisnatural3,
	doi = {10.48550/ARXIV.2301.00601},
	
	url = {https://arxiv.org/abs/2301.00601},
	
	author = {Moshe, Shay Ben},
	
	keywords = {Category Theory (math.CT), Algebraic Topology (math.AT), FOS: Mathematics, FOS: Mathematics},
	
	title = {Naturality of the $\infty$-Categorical Enriched Yoneda Embedding},
	
	publisher = {arXiv},
	
	year = {2023},
	
	copyright = {arXiv.org perpetual, non-exclusive license}
}




@misc{koszulduality,
  doi = {10.48550/ARXIV.1909.11724},
    url = {https://arxiv.org/abs/1909.11724},
    author = {Beardsley, Jonathan and Péroux, Maximilien},
    keywords = {Algebraic Topology (math.AT), Category Theory (math.CT), FOS: Mathematics, FOS: Mathematics, 55U30, 16T15},
    title = {Koszul Duality in Higher Topoi},
    publisher = {arXiv},
    year = {2019},
    copyright = {arXiv.org perpetual, non-exclusive license}
}


@inproceedings {teleman,
    AUTHOR = {Teleman, Constantin},
     TITLE = {Gauge theory and mirror symmetry},
 BOOKTITLE = {Proceedings of the {I}nternational {C}ongress of
              {M}athematicians---{S}eoul 2014. {V}ol. {II}},
     PAGES = {1309--1332},
 PUBLISHER = {Kyung Moon Sa, Seoul},
      YEAR = {2014},
   MRCLASS = {57R56 (18D05 55N91)},
  MRNUMBER = {3728663},
MRREVIEWER = {Ramses Fernandez-Valencia},
}

@misc{PPS_2,
      title={Higher Koszul duality and $n$-affineness}, 
      author={James Pascaleff and Emanuele Pavia and Nicolò Sibilla},
      year={2025},
      eprint={2504.16935},
      archivePrefix={arXiv},
      primaryClass={math.AG},
      url={https://arxiv.org/abs/2504.16935}, 
}

@misc{PPS_1,
      title={Higher local systems and the categorified monodromy equivalence}, 
      author={James Pascaleff and Emanuele Pavia and Nicolò Sibilla},
      year={2025},
      eprint={2501.10241},
      archivePrefix={arXiv},
      primaryClass={math.AT},
      url={https://arxiv.org/abs/2501.10241}, 
}

@book {MR1896125,
    AUTHOR = {Polcino Milies, C\'esar and Sehgal, Sudarshan K.},
     TITLE = {An introduction to group rings},
    SERIES = {Algebra and Applications},
    VOLUME = {1},
 PUBLISHER = {Kluwer Academic Publishers, Dordrecht},
      YEAR = {2002},
     PAGES = {xii+371},
      ISBN = {1-4020-0238-6},
   MRCLASS = {16S34 (16-01 16U60)},
  MRNUMBER = {1896125},
MRREVIEWER = {Edgar\ G.\ Goodaire},
       DOI = {10.1007/978-94-010-0405-3},
       URL = {https://doi.org/10.1007/978-94-010-0405-3},
}


@article {rezk1,
    AUTHOR = {Bergner, Julia E. and Rezk, Charles},
     TITLE = {Comparison of models for {$(\infty,n)$}-categories, {I}},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry \& Topology},
    VOLUME = {17},
      YEAR = {2013},
    NUMBER = {4},
     PAGES = {2163--2202},
      ISSN = {1465-3060},
   MRCLASS = {18D05 (18G55)},
  MRNUMBER = {3109865},
MRREVIEWER = {Javier J. Guti\'{e}rrez},
       DOI = {10.2140/gt.2013.17.2163},
       URL = {https://doi.org/10.2140/gt.2013.17.2163},
}
@article {rezk2,
    AUTHOR = {Bergner, Julia E. and Rezk, Charles},
     TITLE = {Comparison of models for {$(\infty, n)$}-categories, {II}},
   JOURNAL = {J. Topol.},
  FJOURNAL = {Journal of Topology},
    VOLUME = {13},
      YEAR = {2020},
    NUMBER = {4},
     PAGES = {1554--1581},
      ISSN = {1753-8416},
   MRCLASS = {18N65 (18N40 55U35 55U40)},
  MRNUMBER = {4186138},
       DOI = {10.1112/topo.12167},
       URL = {https://doi.org/10.1112/topo.12167},
}


@article {dualizingcartcocart,
	AUTHOR = {Barwick, Clark and Glasman, Saul and Nardin, Denis},
	TITLE = {Dualizing cartesian and cocartesian fibrations},
	JOURNAL = {Theory Appl. Categ.},
	FJOURNAL = {Theory and Applications of Categories},
	VOLUME = {33},
	YEAR = {2018},
	PAGES = {Paper No. 4, 67--94},
	MRCLASS = {18D15},
	MRNUMBER = {3746613},
	MRREVIEWER = {Josep Elgueta},
}


@article {colie,
	AUTHOR = {Ho, Quoc P.},
	TITLE = {Homological stability and densities of generalized
		configuration spaces},
	JOURNAL = {Geom. Topol.},
	FJOURNAL = {Geometry \& Topology},
	VOLUME = {25},
	YEAR = {2021},
	NUMBER = {2},
	PAGES = {813--912},
	ISSN = {1465-3060},
	MRCLASS = {14F35 (14G05 17B62 55P62 55R80)},
	MRNUMBER = {4251437},
	DOI = {10.2140/gt.2021.25.813},
	URL = {https://doi-org.pros1.lib.unimi.it/10.2140/gt.2021.25.813},
}


@incollection {lagcorr,
	AUTHOR = {Calaque, Damien},
	TITLE = {Lagrangian structures on mapping stacks and semi-classical
		{TFT}s},
	BOOKTITLE = {Stacks and categories in geometry, topology, and algebra},
	SERIES = {Contemp. Math.},
	VOLUME = {643},
	PAGES = {1--23},
	PUBLISHER = {Amer. Math. Soc., Providence, RI},
	YEAR = {2015},
	MRCLASS = {53D12 (14A20 14F05 81T45)},
	MRNUMBER = {3381468},
	MRREVIEWER = {Brent Pym},
	DOI = {10.1090/conm/643/12894},
	URL = {https://doi.org/10.1090/conm/643/12894},
}


@article {BRST,
	AUTHOR = {Fuster, Andrea and Henneaux, Marc and Maas, Axel},
	TITLE = {B{RST}-antifield quantization: a short review},
	JOURNAL = {Int. J. Geom. Methods Mod. Phys.},
	FJOURNAL = {International Journal of Geometric Methods in Modern Physics},
	VOLUME = {2},
	YEAR = {2005},
	NUMBER = {5},
	PAGES = {939--963},
	ISSN = {0219-8878},
	MRCLASS = {81T70 (81-02 81T13)},
	MRNUMBER = {2177293},
	MRREVIEWER = {Beatrice Bucker},
	DOI = {10.1142/S0219887805000892},
	URL = {https://doi.org/10.1142/S0219887805000892},
}


@article {BRST2,
	AUTHOR = {Barnich, Glenn and Brandt, Friedemann and Henneaux, Marc},
	TITLE = {Local {BRST} cohomology in gauge theories},
	JOURNAL = {Phys. Rep.},
	FJOURNAL = {Physics Reports. A Review Section of Physics Letters},
	VOLUME = {338},
	YEAR = {2000},
	NUMBER = {5},
	PAGES = {439--569},
	ISSN = {0370-1573},
	MRCLASS = {81T70 (17B81 81-02)},
	MRNUMBER = {1792979},
	MRREVIEWER = {Bani Mitra S\"{o}dermark},
	DOI = {10.1016/S0370-1573(00)00049-1},
	URL = {https://doi.org/10.1016/S0370-1573(00)00049-1},
}


@article {cyclichomology,
	AUTHOR = {Kassel, Christian},
	TITLE = {Cyclic homology, comodules, and mixed complexes},
	JOURNAL = {J. Algebra},
	FJOURNAL = {Journal of Algebra},
	VOLUME = {107},
	YEAR = {1987},
	NUMBER = {1},
	PAGES = {195--216},
	ISSN = {0021-8693},
	MRCLASS = {18G35 (19D55 55U25)},
	MRNUMBER = {883882},
	MRREVIEWER = {Sue Geller},
	DOI = {10.1016/0021-8693(87)90086-X},
	URL = {https://doi-org.pros1.lib.unimi.it/10.1016/0021-8693(87)90086-X},
}


@article {burghelea,
	AUTHOR = {Burghelea, Dan and Ogle, Crichton},
	TITLE = {The {K}\"{u}nneth formula in cyclic homology},
	JOURNAL = {Math. Z.},
	FJOURNAL = {Mathematische Zeitschrift},
	VOLUME = {193},
	YEAR = {1986},
	NUMBER = {4},
	PAGES = {527--536},
	ISSN = {0025-5874},
	MRCLASS = {18F25 (18G15 19D55)},
	MRNUMBER = {867346},
	MRREVIEWER = {Claude Schochet},
	DOI = {10.1007/BF01160473},
	URL = {https://doi-org.pros1.lib.unimi.it/10.1007/BF01160473},
}


@article {coalgebrascomonad,
	AUTHOR = {Hess, Kathryn and Shipley, Brooke},
	TITLE = {The homotopy theory of coalgebras over a comonad},
	JOURNAL = {Proc. Lond. Math. Soc. (3)},
	FJOURNAL = {Proceedings of the London Mathematical Society. Third Series},
	VOLUME = {108},
	YEAR = {2014},
	NUMBER = {2},
	PAGES = {484--516},
	ISSN = {0024-6115},
	MRCLASS = {55U35 (16T15 18C15 18G55 55U15)},
	MRNUMBER = {3166360},
	MRREVIEWER = {Javier J. Guti\'{e}rrez},
	DOI = {10.1112/plms/pdt038},
	URL = {https://doi-org.pros.lib.unimi.it/10.1112/plms/pdt038},
}


@mastersthesis{ozbek,
	title={The Homotopy Theory of Commutative dg Algebras and Representability Theorems for Lie Algebra Cohomology},
	author={Aydin Ozbek},
	year={2016},
	school={University of Nevada, Reno},
%	address={XXX}
}


@article {brown,
	AUTHOR = {Brown, Kenneth S.},
	TITLE = {Abstract homotopy theory and generalized sheaf cohomology},
	JOURNAL = {Trans. Amer. Math. Soc.},
	FJOURNAL = {Transactions of the American Mathematical Society},
	VOLUME = {186},
	YEAR = {1973},
	PAGES = {419--458},
	ISSN = {0002-9947},
	MRCLASS = {55B30 (18H99)},
	MRNUMBER = {341469},
	MRREVIEWER = {A. Dold},
	DOI = {10.2307/1996573},
	URL = {https://doi-org.pros.lib.unimi.it/10.2307/1996573},
}


@misc{hinichdayconvolution,
	doi = {10.48550/ARXIV.2101.09538},
	
	url = {https://arxiv.org/abs/2101.09538},
	
	author = {Hinich, Vladimir},
	
	keywords = {Category Theory (math.CT), Quantum Algebra (math.QA), FOS: Mathematics, FOS: Mathematics, 18D20, 18N60, 18N70},
	
	title = {Colimits in enriched $\infty$-categories and Day convolution},
	
	publisher = {arXiv},
	
	year = {2021},
	
	copyright = {arXiv.org perpetual, non-exclusive license}
}




@article {riehl2,
	AUTHOR = {Riehl, Emily and Verity, Dominic},
	TITLE = {Infinity category theory from scratch},
	JOURNAL = {High. Struct.},
	FJOURNAL = {Higher Structures},
	VOLUME = {4},
	YEAR = {2020},
	NUMBER = {1},
	PAGES = {115--167},
	MRCLASS = {18N60 (18A30 18A40 55U35)},
	MRNUMBER = {4074275},
}

@misc{rezkquasicat,
AUTHOR = {Rezk, Charles},
TITLE = {Introduction to quasicategories},
YEAR={2021},
URL={https://people.math.rochester.edu/faculty/doug/otherpapers/Rezk-quasicats-intro.pdf},
}

@incollection {gepner,
    AUTHOR = {Gepner, David},
     TITLE = {An introduction to higher categorical algebra},
 BOOKTITLE = {Handbook of homotopy theory},
    SERIES = {CRC Press/Chapman Hall Handb. Math. Ser.},
     PAGES = {487--548},
 PUBLISHER = {CRC Press, Boca Raton, FL},
      YEAR = {[2020] \copyright 2020},
      ISBN = {978-0-815-36970-7},
   MRCLASS = {55U35 (16E45 18C10 18C35)},
  MRNUMBER = {4197993},
MRREVIEWER = {Thomas\ H\"uttemann},
}

@article {milnor,
    AUTHOR = {Milnor, John},
     TITLE = {The geometric realization of a semi-simplicial complex},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {65},
      YEAR = {1957},
     PAGES = {357--362},
      ISSN = {0003-486X},
   MRCLASS = {55.0X},
  MRNUMBER = {84138},
MRREVIEWER = {J.\ C.\ Moore},
       DOI = {10.2307/1969967},
       URL = {https://doi.org/10.2307/1969967},
}

@incollection {joyal,
	AUTHOR = {Joyal, A.},
	TITLE = {Quasi-categories and {K}an complexes},
	NOTE = {Special volume celebrating the 70th birthday of Professor Max
		Kelly},
	JOURNAL = {J. Pure Appl. Algebra},
	FJOURNAL = {Journal of Pure and Applied Algebra},
	VOLUME = {175},
	YEAR = {2002},
	NUMBER = {1-3},
	PAGES = {207--222},
	ISSN = {0022-4049},
	MRCLASS = {55U10 (18G55)},
	MRNUMBER = {1935979},
	MRREVIEWER = {Donald M. Davis},
	DOI = {10.1016/S0022-4049(02)00135-4},
	URL = {https://doi-org.pros1.lib.unimi.it/10.1016/S0022-4049(02)00135-4},
}

@book {maysimplicial,
    AUTHOR = {May, J. Peter},
     TITLE = {Simplicial objects in algebraic topology},
    SERIES = {Van Nostrand Mathematical Studies},
    VOLUME = {No. 11},
 PUBLISHER = {D. Van Nostrand Co., Inc., Princeton, N.J.-Toronto,
              Ont.-London},
      YEAR = {1967},
     PAGES = {vi+161},
   MRCLASS = {55.40},
  MRNUMBER = {222892},
MRREVIEWER = {A.\ K.\ Bousfield},
}

@book {riehl3,
	AUTHOR = {Riehl, Emily},
	TITLE = {Categorical homotopy theory},
	SERIES = {New Mathematical Monographs},
	VOLUME = {24},
	PUBLISHER = {Cambridge University Press, Cambridge},
	YEAR = {2014},
	PAGES = {xviii+352},
	ISBN = {978-1-107-04845-4},
	MRCLASS = {18G55 (18D20 55U35)},
	MRNUMBER = {3221774},
	MRREVIEWER = {David A. Blanc},
	DOI = {10.1017/CBO9781107261457},
	URL = {https://doi.org/10.1017/CBO9781107261457},
}


@article {GHN,
	AUTHOR = {Gepner, David and Haugseng, Rune and Nikolaus, Thomas},
	TITLE = {Lax colimits and free fibrations in {$\infty$}-categories},
	JOURNAL = {Doc. Math.},
	FJOURNAL = {Documenta Mathematica},
	VOLUME = {22},
	YEAR = {2017},
	PAGES = {1225--1266},
	ISSN = {1431-0635},
	MRCLASS = {18D30 (18A30)},
	MRNUMBER = {3690268},
	MRREVIEWER = {Josep Elgueta},
}


@misc{laxmonoidal,
	doi = {10.48550/ARXIV.2011.08808},
	
	url = {https://arxiv.org/abs/2011.08808},
	
	author = {Haugseng, Rune and Hebestreit, Fabian and Linskens, Sil and Nuiten, Joost},
	
	keywords = {Category Theory (math.CT), Algebraic Topology (math.AT), FOS: Mathematics, FOS: Mathematics},
	
	title = {Lax monoidal adjunctions, two-variable fibrations and the calculus of mates},
	
	publisher = {arXiv},
	
	year = {2020},
	
	copyright = {arXiv.org perpetual, non-exclusive license}
}


@book {riehlverity,
	AUTHOR = {Riehl, Emily and Verity, Dominic},
	TITLE = {Elements of {$\infty$}-category theory},
	SERIES = {Cambridge Studies in Advanced Mathematics},
	VOLUME = {194},
	PUBLISHER = {Cambridge University Press, Cambridge},
	YEAR = {2022},
	PAGES = {xix+759},
	ISBN = {978-1-108-83798-9},
	MRCLASS = {18-02 (18Nxx)},
	MRNUMBER = {4354541},
	DOI = {10.1017/9781108936880},
	URL = {https://doi.org/10.1017/9781108936880},
}


@article {riehl,
	AUTHOR = {Ching, Michael and Riehl, Emily},
	TITLE = {Coalgebraic models for combinatorial model categories},
	JOURNAL = {Homology Homotopy Appl.},
	FJOURNAL = {Homology, Homotopy and Applications},
	VOLUME = {16},
	YEAR = {2014},
	NUMBER = {2},
	PAGES = {171--184},
	ISSN = {1532-0073},
	MRCLASS = {18C35},
	MRNUMBER = {3257572},
	MRREVIEWER = {George Ciprian Modoi},
	DOI = {10.4310/HHA.2014.v16.n2.a9},
	URL = {https://doi.org/10.4310/HHA.2014.v16.n2.a9},
}


@misc{derivedfoliations2,
	title={Algebraic foliations and derived geometry II: the Grothendieck-Riemann-Roch theorem},
	author={Bertrand Toën and Gabriele Vezzosi},
	year={2020},
	eprint={2007.09251},
	archivePrefix={arXiv},
	primaryClass={math.AG}
}


@misc{toen2020algebraic,
	title={Algebraic foliations and derived geometry I: the Riemann-Hilbert correspondence}, 
	author={Bertrand Toën and Gabriele Vezzosi},
	year={2020},
	eprint={2001.05450},
	archivePrefix={arXiv},
	primaryClass={math.AG}
}


@article {krizmay,
	AUTHOR = {K\v{r}\'{\i}\v{z}, Igor and May, J. P.},
	TITLE = {Operads, algebras, modules and motives},
	JOURNAL = {Ast\'{e}risque},
	FJOURNAL = {Ast\'{e}risque},
	NUMBER = {233},
	YEAR = {1995},
	PAGES = {iv+145pp},
	ISSN = {0303-1179},
	MRCLASS = {18G99 (14F99 19E99 55U99)},
	MRNUMBER = {1361938},
	MRREVIEWER = {J. P. C. Greenlees},
}


@article {dwyerkan,
	AUTHOR = {Dwyer, W. G. and Kan, D. M.},
	TITLE = {Calculating simplicial localizations},
	JOURNAL = {J. Pure Appl. Algebra},
	FJOURNAL = {Journal of Pure and Applied Algebra},
	VOLUME = {18},
	YEAR = {1980},
	NUMBER = {1},
	PAGES = {17--35},
	ISSN = {0022-4049},
	MRCLASS = {55U35 (18D20)},
	MRNUMBER = {578563},
	MRREVIEWER = {Timothy Porter},
	DOI = {10.1016/0022-4049(80)90113-9},
	URL = {https://doi-org.pros.lib.unimi.it/10.1016/0022-4049(80)90113-9},
}


@article {ching,
	AUTHOR = {Ching, Michael},
	TITLE = {Bar-cobar duality for operads in stable homotopy theory},
	JOURNAL = {J. Topol.},
	FJOURNAL = {Journal of Topology},
	VOLUME = {5},
	YEAR = {2012},
	NUMBER = {1},
	PAGES = {39--80},
	ISSN = {1753-8416},
	MRCLASS = {55P48 (18D50 55P42)},
	MRNUMBER = {2897049},
	MRREVIEWER = {Beno\^{\i}t Fresse},
	DOI = {10.1112/jtopol/jtr027},
	URL = {https://doi-org.pros.lib.unimi.it/10.1112/jtopol/jtr027},
}


@article {baranovsky,
	AUTHOR = {Baranovsky, Vladimir},
	TITLE = {A universal enveloping for {$L_\infty$}-algebras},
	JOURNAL = {Math. Res. Lett.},
	FJOURNAL = {Mathematical Research Letters},
	VOLUME = {15},
	YEAR = {2008},
	NUMBER = {6},
	PAGES = {1073--1089},
	ISSN = {1073-2780},
	MRCLASS = {18G55 (17B55)},
	MRNUMBER = {2470385},
	MRREVIEWER = {Wendy Lowen},
	DOI = {10.4310/MRL.2008.v15.n6.a1},
	URL = {https://doi-org.pros.lib.unimi.it/10.4310/MRL.2008.v15.n6.a1},
}


@article {modelstructureforgoldmanmillson,
	AUTHOR = {Robert-Nicoud, Daniel},
	TITLE = {A model structure for the {G}oldman-{M}illson theorem},
	JOURNAL = {Grad. J. Math.},
	FJOURNAL = {The Graduate Journal of Mathematics},
	VOLUME = {3},
	YEAR = {2018},
	NUMBER = {1},
	PAGES = {15--30},
	MRCLASS = {18G55 (17B55)},
	MRNUMBER = {3876592},
	MRREVIEWER = {Zuhier Khaled Altawallbeh},
}


@article {stronglyhomotopyliealgebras,
	AUTHOR = {Lada, Tom and Markl, Martin},
	TITLE = {Strongly homotopy {L}ie algebras},
	JOURNAL = {Comm. Algebra},
	FJOURNAL = {Communications in Algebra},
	VOLUME = {23},
	YEAR = {1995},
	NUMBER = {6},
	PAGES = {2147--2161},
	ISSN = {0092-7872},
	MRCLASS = {16S30 (17B35 18G99)},
	MRNUMBER = {1327129},
	MRREVIEWER = {Stanis\l aw Betley},
	DOI = {10.1080/00927879508825335},
	URL = {https://doi-org.pros.lib.unimi.it/10.1080/00927879508825335},
}


@article {linearbatalin,
	AUTHOR = {Gwilliam, Owen and Haugseng, Rune},
	TITLE = {Linear {B}atalin-{V}ilkovisky quantization as a functor of
		{$\infty$}-categories},
	JOURNAL = {Selecta Math. (N.S.)},
	FJOURNAL = {Selecta Mathematica. New Series},
	VOLUME = {24},
	YEAR = {2018},
	NUMBER = {2},
	PAGES = {1247--1313},
	ISSN = {1022-1824},
	MRCLASS = {18G55 (14D23 17B37 18D50 53D55 58J52 81Q99 81T70)},
	MRNUMBER = {3782422},
	MRREVIEWER = {Olga Kravchenko},
	DOI = {10.1007/s00029-018-0396-0},
	URL = {https://doi-org.pros.lib.unimi.it/10.1007/s00029-018-0396-0},
}


@article {chiralkoszul,
	AUTHOR = {Francis, John and Gaitsgory, Dennis},
	TITLE = {Chiral {K}oszul duality},
	JOURNAL = {Selecta Math. (N.S.)},
	FJOURNAL = {Selecta Mathematica. New Series},
	VOLUME = {18},
	YEAR = {2012},
	NUMBER = {1},
	PAGES = {27--87},
	ISSN = {1022-1824},
	MRCLASS = {14F10 (14F05 14H81 17B55 18D10 18D50)},
	MRNUMBER = {2891861},
	MRREVIEWER = {Beno\^{\i}t Fresse},
	DOI = {10.1007/s00029-011-0065-z},
	URL = {https://doi.org/10.1007/s00029-011-0065-z},
}


@article {rationalhomotopytheory,
	AUTHOR = {Quillen, Daniel},
	TITLE = {Rational homotopy theory},
	JOURNAL = {Ann. of Math. (2)},
	FJOURNAL = {Annals of Mathematics. Second Series},
	VOLUME = {90},
	YEAR = {1969},
	PAGES = {205--295},
	ISSN = {0003-486X},
	MRCLASS = {55.40},
	MRNUMBER = {258031},
	MRREVIEWER = {J. F. Adams},
	DOI = {10.2307/1970725},
	URL = {https://doi-org.pros.lib.unimi.it/10.2307/1970725},
}


@article {priddykoszul,
    AUTHOR = {Priddy, Stewart B.},
     TITLE = {Koszul resolutions},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {152},
      YEAR = {1970},
     PAGES = {39--60},
      ISSN = {0002-9947,1088-6850},
   MRCLASS = {18.20},
  MRNUMBER = {265437},
MRREVIEWER = {A.\ K.\ Bousfield},
       DOI = {10.2307/1995637},
       URL = {https://doi.org/10.2307/1995637},
}


@article {enhancingfiltered,
	AUTHOR = {Gwilliam, Owen and Pavlov, Dmitri},
	TITLE = {Enhancing the filtered derived category},
	JOURNAL = {J. Pure Appl. Algebra},
	FJOURNAL = {Journal of Pure and Applied Algebra},
	VOLUME = {222},
	YEAR = {2018},
	NUMBER = {11},
	PAGES = {3621--3674},
	ISSN = {0022-4049},
	MRCLASS = {18E30 (18E10)},
	MRNUMBER = {3806745},
	MRREVIEWER = {Wolfgang Rump},
	DOI = {10.1016/j.jpaa.2018.01.004},
	URL = {https://doi-org.pros.lib.unimi.it:2050/10.1016/j.jpaa.2018.01.004},
}


@book {quillenhomotopicalalgebra,
	AUTHOR = {Quillen, Daniel G.},
	TITLE = {Homotopical algebra},
	SERIES = {Lecture Notes in Mathematics, No. 43},
	PUBLISHER = {Springer-Verlag, Berlin-New York},
	YEAR = {1967},
	PAGES = {iv+156 pp. (not consecutively paged)},
	MRCLASS = {18.20 (55.00)},
	MRNUMBER = {0223432},
	MRREVIEWER = {A. K. Bousfield},
}


@book {MR0420609,
	AUTHOR = {Boardman, J. M. and Vogt, R. M.},
	TITLE = {Homotopy invariant algebraic structures on topological spaces},
	SERIES = {Lecture Notes in Mathematics, Vol. 347},
	PUBLISHER = {Springer-Verlag, Berlin-New York},
	YEAR = {1973},
	PAGES = {x+257},
	MRCLASS = {55D35},
	MRNUMBER = {0420609},
	MRREVIEWER = {J. Stasheff},
}


@article {rezk,
	AUTHOR = {Rezk, Charles},
	TITLE = {A model for the homotopy theory of homotopy theory},
	JOURNAL = {Trans. Amer. Math. Soc.},
	FJOURNAL = {Transactions of the American Mathematical Society},
	VOLUME = {353},
	YEAR = {2001},
	NUMBER = {3},
	PAGES = {973--1007},
	ISSN = {0002-9947},
	MRCLASS = {55U35 (18G30)},
	MRNUMBER = {1804411},
	MRREVIEWER = {Brooke E. Shipley},
	DOI = {10.1090/S0002-9947-00-02653-2},
	URL = {https://doi-org.pros1.lib.unimi.it/10.1090/S0002-9947-00-02653-2},
}


@article {albrechtpuppe,
	AUTHOR = {Dold, Albrecht and Puppe, Dieter},
	TITLE = {Homologie nicht-additiver {F}unktoren. {A}nwendungen},
	JOURNAL = {Ann. Inst. Fourier (Grenoble)},
	FJOURNAL = {Universit\'{e} de Grenoble. Annales de l'Institut Fourier},
	VOLUME = {11},
	YEAR = {1961},
	PAGES = {201--312},
	ISSN = {0373-0956},
	MRCLASS = {18.20},
	MRNUMBER = {150183},
	MRREVIEWER = {P. J. Hilton},
	URL = {http://www.numdam.org/item?id=AIF_1961__11__201_0},
}


@article {nuiten19,
	AUTHOR = {Nuiten, Joost},
	TITLE = {Homotopical algebra for {L}ie algebroids},
	JOURNAL = {Appl. Categ. Structures},
	FJOURNAL = {Applied Categorical Structures. A Journal Devoted to
		Applications of Categorical Methods in Algebra, Analysis,
		Order, Topology and Computer Science},
	VOLUME = {27},
	YEAR = {2019},
	NUMBER = {5},
	PAGES = {493--534},
	ISSN = {0927-2852},
	MRCLASS = {18G55 (55U15 55U35)},
	MRNUMBER = {4003715},
	MRREVIEWER = {Hirokazu Nishimura},
	DOI = {10.1007/s10485-019-09563-z},
	URL = {https://doi-org.pros2.lib.unimi.it/10.1007/s10485-019-09563-z},
}


@article {BMS,
    AUTHOR = {Bhatt, Bhargav and Morrow, Matthew and Scholze, Peter},
     TITLE = {Topological {H}ochschild homology and integral {$p$}-adic
              {H}odge theory},
   JOURNAL = {Publ. Math. Inst. Hautes \'{E}tudes Sci.},
  FJOURNAL = {Publications Math\'{e}matiques. Institut de Hautes \'{E}tudes
              Scientifiques},
    VOLUME = {129},
      YEAR = {2019},
     PAGES = {199--310},
      ISSN = {0073-8301},
   MRCLASS = {14F30 (13A35)},
  MRNUMBER = {3949030},
       DOI = {10.1007/s10240-019-00106-9},
       URL = {https://doi-org.pros.lib.unimi.it:2050/10.1007/s10240-019-00106-9},
}


@article {integraltransforms,
    AUTHOR = {Ben-Zvi, David and Francis, John and Nadler, David},
     TITLE = {Integral transforms and {D}rinfeld centers in derived
              algebraic geometry},
   JOURNAL = {J. Amer. Math. Soc.},
  FJOURNAL = {Journal of the American Mathematical Society},
    VOLUME = {23},
      YEAR = {2010},
    NUMBER = {4},
     PAGES = {909--966},
      ISSN = {0894-0347,1088-6834},
   MRCLASS = {14D23 (14F05 18D10 18E30)},
  MRNUMBER = {2669705},
MRREVIEWER = {Andrei\ D.\ Halanay},
       DOI = {10.1090/S0894-0347-10-00669-7},
       URL = {https://doi.org/10.1090/S0894-0347-10-00669-7},
}


@article {indcoh,
    AUTHOR = {Gaitsgory, Dennis},
     TITLE = {ind-coherent sheaves},
   JOURNAL = {Mosc. Math. J.},
  FJOURNAL = {Moscow Mathematical Journal},
    VOLUME = {13},
      YEAR = {2013},
    NUMBER = {3},
     PAGES = {399--528, 553},
      ISSN = {1609-3321},
   MRCLASS = {14F05 (14D24)},
  MRNUMBER = {3136100},
MRREVIEWER = {Cristian V. Anghel},
       DOI = {10.17323/1609-4514-2013-13-3-399-528},
       URL = {https://doi.org/10.17323/1609-4514-2013-13-3-399-528},
}


@book {serre,
	AUTHOR = {Serre, Jean-Pierre},
	TITLE = {Alg\`ebre locale. {M}ultiplicit\'{e}s},
	SERIES = {Lecture Notes in Mathematics},
	VOLUME = {11},
	NOTE = {Cours au Coll\`ege de France, 1957--1958, r\'{e}dig\'{e} par Pierre
		Gabriel,
		Seconde \'{e}dition, 1965},
	PUBLISHER = {Springer-Verlag, Berlin-New York},
	YEAR = {1965},
	PAGES = {vii+188 pp. (not consecutively paged)},
	MRCLASS = {13.95 (14.08)},
	MRNUMBER = {0201468},
	MRREVIEWER = {M. Nagata},
}


@misc{UHKR,
    title={A Universal HKR Theorem},
    author={Tasos Moulinos and Marco Robalo and Bertrand Toën},
    year={2019},
    eprint={1906.00118},
    archivePrefix={arXiv},
    primaryClass={math.AG}
}


@article {thetaspace,
    AUTHOR = {Rezk, Charles},
     TITLE = {A {C}artesian presentation of weak {$n$}-categories},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry \& Topology},
    VOLUME = {14},
      YEAR = {2010},
    NUMBER = {1},
     PAGES = {521--571},
      ISSN = {1465-3060},
   MRCLASS = {18D05 (55U40)},
  MRNUMBER = {2578310},
       DOI = {10.2140/gt.2010.14.521},
       URL = {https://doi.org/10.2140/gt.2010.14.521},
}


@article {enrichment,
    AUTHOR = {Heine, Hadrian},
     TITLE = {An equivalence between two models of {$\infty $}-categories of
              enriched presheaves},
   JOURNAL = {Appl. Categ. Structures},
  FJOURNAL = {Applied Categorical Structures. A Journal Devoted to
              Applications of Categorical Methods in Algebra, Analysis,
              Computer Science, Logic, Order and Topology},
    VOLUME = {33},
      YEAR = {2025},
    NUMBER = {1},
     PAGES = {Paper No. 2, 19},
      ISSN = {0927-2852,1572-9095},
   MRCLASS = {18N65 (18N70)},
  MRNUMBER = {4832426},
       DOI = {10.1007/s10485-024-09792-x},
       URL = {https://doi.org/10.1007/s10485-024-09792-x},
}

@article {hoyois_quadratic_refinement,
    AUTHOR = {Hoyois, Marc},
     TITLE = {A quadratic refinement of the
              {G}rothendieck-{L}efschetz-{V}erdier trace formula},
   JOURNAL = {Algebr. Geom. Topol.},
  FJOURNAL = {Algebraic \& Geometric Topology},
    VOLUME = {14},
      YEAR = {2014},
    NUMBER = {6},
     PAGES = {3603--3658},
      ISSN = {1472-2747,1472-2739},
   MRCLASS = {14F42 (11E81 55M20)},
  MRNUMBER = {3302973},
MRREVIEWER = {Daniel\ C.\ Isaksen},
       DOI = {10.2140/agt.2014.14.3603},
       URL = {https://doi.org/10.2140/agt.2014.14.3603},
}

@misc{Clausen_Scholze_lectures, 
author = {Clausen, Dustin and Scholze, Peter},
title = {Analytic stacks},
howpublished = "\url{https://www.youtube.com/watch?v=YxSZ1mTIpaA}",
year = {2024}, 
note = "Accessed 05/05/2025",
}


@article {thetaspaceerr,
    AUTHOR = {Rezk, Charles},
     TITLE = {Correction to ``{A} {C}artesian presentation of weak
              {$n$}-categories''},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry \& Topology},
    VOLUME = {14},
      YEAR = {2010},
    NUMBER = {4},
     PAGES = {2301--2304},
      ISSN = {1465-3060,1364-0380},
   MRCLASS = {18D05 (55U40)},
  MRNUMBER = {2740648},
       DOI = {10.2140/gt.2010.14.2301},
       URL = {https://doi.org/10.2140/gt.2010.14.2301},
}


@article {kellerhochschildhomology,
    AUTHOR = {Keller, Bernhard},
     TITLE = {On the cyclic homology of ringed spaces and schemes},
   JOURNAL = {Doc. Math.},
  FJOURNAL = {Documenta Mathematica},
    VOLUME = {3},
      YEAR = {1998},
     PAGES = {231--259},
      ISSN = {1431-0635},
   MRCLASS = {16E40 (14F05 18E30)},
  MRNUMBER = {1647519},
MRREVIEWER = {Kevin P. Knudson},
}


@incollection {preygel,
    AUTHOR = {Preygel, Anatoly},
     TITLE = {Ind-coherent complexes on loop spaces and connections},
 BOOKTITLE = {Stacks and categories in geometry, topology, and algebra},
    SERIES = {Contemp. Math.},
    VOLUME = {643},
     PAGES = {289--323},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2015},
   MRCLASS = {14F05 (14F10 14F40)},
  MRNUMBER = {3381476},
MRREVIEWER = {Andreas H\"{o}ring},
       DOI = {10.1090/conm/643/12902},
       URL = {https://doi.org/10.1090/conm/643/12902},
}


@incollection {simpson,
    AUTHOR = {Simpson, Carlos},
     TITLE = {The {H}odge filtration on nonabelian cohomology},
 BOOKTITLE = {Algebraic geometry---{S}anta {C}ruz 1995},
    SERIES = {Proc. Sympos. Pure Math.},
    VOLUME = {62},
     PAGES = {217--281},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {1997},
   MRCLASS = {14F99 (14C30 14D20 32J25 32J27 53C55)},
  MRNUMBER = {1492538},
MRREVIEWER = {Nitin Nitsure},
       DOI = {10.1090/pspum/062.2/1492538},
       URL = {https://doi.org/10.1090/pspum/062.2/1492538},
}


@misc{benzvi2012morita,
      title={Morita equivalence for convolution categories: Appendix to arXiv:0805.0157}, 
      author={David Ben-Zvi and John Francis and David Nadler},
      year={2012},
      eprint={1209.0193},
      archivePrefix={arXiv},
      primaryClass={math.AG}
}


@article {BZN,
    AUTHOR = {Ben-Zvi, David and Nadler, David},
     TITLE = {Loop spaces and connections},
   JOURNAL = {J. Topol.},
  FJOURNAL = {Journal of Topology},
    VOLUME = {5},
      YEAR = {2012},
    NUMBER = {2},
     PAGES = {377--430},
      ISSN = {1753-8416},
   MRCLASS = {14F05 (14F10 19D55 55P35)},
  MRNUMBER = {2928082},
MRREVIEWER = {Julia Bergner},
       DOI = {10.1112/jtopol/jts007},
       URL = {https://doi.org/10.1112/jtopol/jts007},
}


@article {HKRTV,
    AUTHOR = {To\"{e}n, Bertrand and Vezzosi, Gabriele},
     TITLE = {Alg\`ebres simpliciales {$S^1$}-\'{e}quivariantes, th\'{e}orie de de
              {R}ham et th\'{e}or\`emes {HKR} multiplicatifs},
   JOURNAL = {Compos. Math.},
  FJOURNAL = {Compositio Mathematica},
    VOLUME = {147},
      YEAR = {2011},
    NUMBER = {6},
     PAGES = {1979--2000},
      ISSN = {0010-437X},
   MRCLASS = {18G55 (14F40 16E45 18G30 55U10)},
  MRNUMBER = {2862069},
MRREVIEWER = {Kenneth A. Brown},
       DOI = {10.1112/S0010437X11005501},
       URL = {https://doi.org/10.1112/S0010437X11005501},
}


@incollection {gwtheory,
    AUTHOR = {Rose, Simon C. F.},
     TITLE = {Introduction to {G}romov-{W}itten theory},
 BOOKTITLE = {Calabi-{Y}au varieties: arithmetic, geometry and physics},
    SERIES = {Fields Inst. Monogr.},
    VOLUME = {34},
     PAGES = {281--301},
 PUBLISHER = {Fields Inst. Res. Math. Sci., Toronto, ON},
      YEAR = {2015},
   MRCLASS = {14N35 (53D45)},
  MRNUMBER = {3409778},
MRREVIEWER = {Hsian-Hua Tseng},
       DOI = {10.1007/978-1-4939-2830-9_8},
       URL = {https://doi.org/10.1007/978-1-4939-2830-9_8},
}




@misc{hoyois2018categorified,
    title={The categorified Grothendieck-Riemann-Roch theorem},
    author={Marc Hoyois and Pavel Safronov and Sarah Scherotzke and Nicolò Sibilla},
    year={2018},
    eprint={1804.00879},
    archivePrefix={arXiv},
    primaryClass={math.KT}
}


@article {GR,
    AUTHOR = {Gaitsgory, Dennis and Rozenblyum, Nick},
     TITLE = {Crystals and {D}-modules},
   JOURNAL = {Pure Appl. Math. Q.},
  FJOURNAL = {Pure and Applied Mathematics Quarterly},
    VOLUME = {10},
      YEAR = {2014},
    NUMBER = {1},
     PAGES = {57--154},
      ISSN = {1558-8599},
   MRCLASS = {14A20 (14F05 14F10)},
  MRNUMBER = {3264953},
MRREVIEWER = {Andrei D. Halanay},
       DOI = {10.4310/PAMQ.2014.v10.n1.a2},
       URL = {https://doi.org/10.4310/PAMQ.2014.v10.n1.a2},
}


@article {barannikov,
    AUTHOR = {Barannikov, Serguei},
     TITLE = {Quantum periods. {I}. {S}emi-infinite variations of {H}odge
              structures},
   JOURNAL = {Internat. Math. Res. Notices},
  FJOURNAL = {International Mathematics Research Notices},
      YEAR = {2001},
    NUMBER = {23},
     PAGES = {1243--1264},
      ISSN = {1073-7928},
   MRCLASS = {32G20 (14D07 14J32 32J25 32Q25)},
  MRNUMBER = {1866443},
MRREVIEWER = {Gregory J. Pearlstein},
       DOI = {10.1155/S1073792801000599},
       URL = {https://doi.org/10.1155/S1073792801000599},
}


@article {mukaipairing,
    AUTHOR = {C\u{a}ld\u{a}raru, Andrei},
     TITLE = {The {M}ukai pairing. {II}. {T}he
              {H}ochschild-{K}ostant-{R}osenberg isomorphism},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {194},
      YEAR = {2005},
    NUMBER = {1},
     PAGES = {34--66},
      ISSN = {0001-8708},
   MRCLASS = {14F40 (19L10)},
  MRNUMBER = {2141853},
MRREVIEWER = {David Ploog},
       DOI = {10.1016/j.aim.2004.05.012},
       URL = {https://doi.org/10.1016/j.aim.2004.05.012},
}


@misc{sheridanncht,
    title={Formulae in noncommutative Hodge theory},
    author={Nick Sheridan},
    year={2015},
    eprint={1510.03795},
    archivePrefix={arXiv},
    primaryClass={math.KT}
}


@article {GMconnection,
    AUTHOR = {Katz, Nicholas M. and Oda, Tadao},
     TITLE = {On the differentiation of de {R}ham cohomology classes with
              respect to parameters},
   JOURNAL = {J. Math. Kyoto Univ.},
  FJOURNAL = {Journal of Mathematics of Kyoto University},
    VOLUME = {8},
      YEAR = {1968},
     PAGES = {199--213},
      ISSN = {0023-608X},
   MRCLASS = {14.52},
  MRNUMBER = {237510},
MRREVIEWER = {James Milne},
       DOI = {10.1215/kjm/1250524135},
       URL = {https://doi.org/10.1215/kjm/1250524135},
}


@article {shklyarov,
    AUTHOR = {Shklyarov, Dmytro},
     TITLE = {Matrix factorizations and higher residue pairings},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {292},
      YEAR = {2016},
     PAGES = {181--209},
      ISSN = {0001-8708},
   MRCLASS = {14A22 (16E40 16E45 18D10 32S50)},
  MRNUMBER = {3464022},
MRREVIEWER = {Andrea Solotar},
       DOI = {10.1016/j.aim.2016.01.014},
       URL = {https://doi.org/10.1016/j.aim.2016.01.014},
}


@incollection {getzler,
    AUTHOR = {Getzler, Ezra},
     TITLE = {Cartan homotopy formulas and the {G}auss-{M}anin connection in
              cyclic homology},
 BOOKTITLE = {Quantum deformations of algebras and their representations
              ({R}amat-{G}an, 1991/1992; {R}ehovot, 1991/1992)},
    SERIES = {Israel Math. Conf. Proc.},
    VOLUME = {7},
     PAGES = {65--78},
 PUBLISHER = {Bar-Ilan Univ., Ramat Gan},
      YEAR = {1993},
   MRCLASS = {19D55 (18G60 53C05)},
  MRNUMBER = {1261901},
MRREVIEWER = {Ulrike Tillmann},
}


@article {highertraces,
	AUTHOR = {Hoyois, Marc and Scherotzke, Sarah and Sibilla, Nicol\`o},
	TITLE = {Higher traces, noncommutative motives, and the categorified
		{C}hern character},
	JOURNAL = {Adv. Math.},
	FJOURNAL = {Advances in Mathematics},
	VOLUME = {309},
	YEAR = {2017},
	PAGES = {97--154},
	ISSN = {0001-8708},
	MRCLASS = {14F05 (14F42 18D05 19D55)},
	MRNUMBER = {3607274},
	MRREVIEWER = {Satoshi Mochizuki},
	DOI = {10.1016/j.aim.2017.01.008},
	URL = {https://doi.org/10.1016/j.aim.2017.01.008},
}


@article {eilenbergmoorespectralsequence,
	AUTHOR = {Eilenberg, Samuel and Moore, John C.},
	TITLE = {Homology and fibrations. {I}. {C}oalgebras, cotensor product
		and its derived functors},
	JOURNAL = {Comment. Math. Helv.},
	FJOURNAL = {Commentarii Mathematici Helvetici},
	VOLUME = {40},
	YEAR = {1966},
	PAGES = {199--236},
	ISSN = {0010-2571},
	MRCLASS = {55.50},
	MRNUMBER = {203730},
	MRREVIEWER = {A. Heller},
	DOI = {10.1007/BF02564371},
	URL = {https://doi.org/10.1007/BF02564371},
}


@article {koszuldualitypatterns,
	AUTHOR = {Beilinson, Alexander and Ginzburg, Victor and Soergel,
		Wolfgang},
	TITLE = {Koszul duality patterns in representation theory},
	JOURNAL = {J. Amer. Math. Soc.},
	FJOURNAL = {Journal of the American Mathematical Society},
	VOLUME = {9},
	YEAR = {1996},
	NUMBER = {2},
	PAGES = {473--527},
	ISSN = {0894-0347},
	MRCLASS = {17B10 (14F10 16W50)},
	MRNUMBER = {1322847},
	MRREVIEWER = {Rolf K\"{a}llstr\"{o}m},
	DOI = {10.1090/S0894-0347-96-00192-0},
	URL = {https://doi.org/10.1090/S0894-0347-96-00192-0},
}


@article {arinkingaitsgory,
	AUTHOR = {Arinkin, D. and Gaitsgory, D.},
	TITLE = {Singular support of coherent sheaves and the geometric
		{L}anglands conjecture},
	JOURNAL = {Selecta Math. (N.S.)},
	FJOURNAL = {Selecta Mathematica. New Series},
	VOLUME = {21},
	YEAR = {2015},
	NUMBER = {1},
	PAGES = {1--199},
	ISSN = {1022-1824},
	MRCLASS = {14D24 (14A20 14F05 22E57)},
	MRNUMBER = {3300415},
	MRREVIEWER = {Richard P. Thomas},
	DOI = {10.1007/s00029-014-0167-5},
	URL = {https://doi.org/10.1007/s00029-014-0167-5},
}


@article {haineportateyssier,
    AUTHOR = {Haine, Peter J. and Porta, Mauro and Teyssier, Jean-Baptiste},
     TITLE = {The homotopy-invariance of constructible sheaves},
   JOURNAL = {Homology Homotopy Appl.},
  FJOURNAL = {Homology, Homotopy and Applications},
    VOLUME = {25},
      YEAR = {2023},
    NUMBER = {2},
     PAGES = {97--128},
      ISSN = {1532-0073,1532-0081},
   MRCLASS = {55N30 (18F20 32S60 55N05 55P55)},
  MRNUMBER = {4651175},
       DOI = {10.4310/hha.2023.v25.n2.a6},
       URL = {https://doi.org/10.4310/hha.2023.v25.n2.a6},
}


@misc{symmetricspectra,
AUTHOR = {Schwede, Stefan},
TITLE = {Symmetric Spectra},
YEAR = {2012},
URL ={http://www.math.uni-bonn.de/people/schwede/SymSpec-v3.pdf}
}

@misc{khan_notes,
AUTHOR = {Khan, Adeel A.},
TITLE = {An introduction to derived algebraic geometry},
YEAR={2023},
URL={https://www.preschema.com/lecture-notes/2023-kias/dagkias.pdf}
}

@article {dwyerduality,
	AUTHOR = {Dwyer, W. G. and Greenlees, J. P. C. and Iyengar, S.},
	TITLE = {Duality in algebra and topology},
	JOURNAL = {Adv. Math.},
	FJOURNAL = {Advances in Mathematics},
	VOLUME = {200},
	YEAR = {2006},
	NUMBER = {2},
	PAGES = {357--402},
	ISSN = {0001-8708},
	MRCLASS = {55P43 (13H10 16D90 18E30 55R40 57N65)},
	MRNUMBER = {2200850},
	MRREVIEWER = {Andrey Yu. Lazarev},
	DOI = {10.1016/j.aim.2005.11.004},
	URL = {https://doi-org.pros1.lib.unimi.it/10.1016/j.aim.2005.11.004},
}


@article {rothenbergsteenrod,
	AUTHOR = {Rothenberg, M. and Steenrod, N. E.},
	TITLE = {The cohomology of classifying spaces of {$H$}-spaces},
	JOURNAL = {Bull. Amer. Math. Soc.},
	FJOURNAL = {Bulletin of the American Mathematical Society},
	VOLUME = {71},
	YEAR = {1965},
	PAGES = {872--875},
	ISSN = {0002-9904},
	MRCLASS = {55.40},
	MRNUMBER = {208596},
	MRREVIEWER = {A. Dold},
	DOI = {10.1090/S0002-9904-1965-11420-3},
	URL = {https://doi-org.pros1.lib.unimi.it/10.1090/S0002-9904-1965-11420-3},
}


@incollection {perversesheaves,
	AUTHOR = {Be\u{\i}linson, A. A. and Bernstein, J. and Deligne, P.},
	TITLE = {Faisceaux pervers},
	BOOKTITLE = {Analysis and topology on singular spaces, {I} ({L}uminy,
		1981)},
	SERIES = {Ast\'{e}risque},
	VOLUME = {100},
	PAGES = {5--171},
	PUBLISHER = {Soc. Math. France, Paris},
	YEAR = {1982},
	MRCLASS = {32C38},
	MRNUMBER = {751966},
	MRREVIEWER = {Zoghman Mebkhout},
}


@book {mccleary,
    AUTHOR = {McCleary, John},
     TITLE = {A user's guide to spectral sequences},
    SERIES = {Cambridge Studies in Advanced Mathematics},
    VOLUME = {58},
   EDITION = {Second},
 PUBLISHER = {Cambridge University Press, Cambridge},
      YEAR = {2001},
     PAGES = {xvi+561},
      ISBN = {0-521-56759-9},
   MRCLASS = {55Txx (18G40)},
  MRNUMBER = {1793722},
MRREVIEWER = {Frank\ Neumann},
}


@incollection {1affineness,
	AUTHOR = {Gaitsgory, Dennis},
	TITLE = {Sheaves of categories and the notion of 1-affineness},
	BOOKTITLE = {Stacks and categories in geometry, topology, and algebra},
	SERIES = {Contemp. Math.},
	VOLUME = {643},
	PAGES = {127--225},
	PUBLISHER = {Amer. Math. Soc., Providence, RI},
	YEAR = {2015},
	MRCLASS = {14F05 (14A20)},
	MRNUMBER = {3381473},
	MRREVIEWER = {Jon Eivind Vatne},
	DOI = {10.1090/conm/643/12899},
	URL = {https://doi.org/10.1090/conm/643/12899},
}


@article {beke,
	AUTHOR = {Beke, Tibor},
	TITLE = {Sheafifiable homotopy model categories},
	JOURNAL = {Math. Proc. Cambridge Philos. Soc.},
	FJOURNAL = {Mathematical Proceedings of the Cambridge Philosophical
		Society},
	VOLUME = {129},
	YEAR = {2000},
	NUMBER = {3},
	PAGES = {447--475},
	ISSN = {0305-0041},
	MRCLASS = {18D15 (03C95 18F20 18G55)},
	MRNUMBER = {1780498},
	MRREVIEWER = {Masahiko Niwa},
	DOI = {10.1017/S0305004100004722},
	URL = {https://doi.org/10.1017/S0305004100004722},
}


@misc{stefanich2020presentable,
	title={Presentable $(\infty, n)$-categories}, 
	author={Germán Stefanich},
	year={2020},
	eprint={2011.03035},
	archivePrefix={arXiv},
	primaryClass={math.AT}
}
@book {stefanichthesis,
    AUTHOR = {Stefanich, German},
     TITLE = {Higher {Q}uasicoherent {S}heaves},
      NOTE = {Thesis (Ph.D.)--University of California, Berkeley},
 PUBLISHER = {ProQuest LLC, Ann Arbor, MI},
      YEAR = {2021},
     PAGES = {347},
      ISBN = {979-8535-56467-8},
   MRCLASS = {99-05},
  MRNUMBER = {4326588},
       URL =
              {http://gateway.proquest.com/openurl?url_ver=Z39.88-2004&rft_val_fmt=info:ofi/fmt:kev:mtx:dissertation&res_dat=xri:pqm&rft_dat=xri:pqdiss:28540389},
}


@article {iwanari,
	AUTHOR = {Iwanari, Isamu},
	TITLE = {Differential calculus of {H}ochschild pairs for
		infinity-categories},
	JOURNAL = {SIGMA Symmetry Integrability Geom. Methods Appl.},
	FJOURNAL = {SIGMA. Symmetry, Integrability and Geometry. Methods and
		Applications},
	VOLUME = {16},
	YEAR = {2020},
	PAGES = {Paper No. 097, 57},
	MRCLASS = {16E40 (18M60 18N60)},
	MRNUMBER = {4156865},
	MRREVIEWER = {Beno\^{\i}t Fresse},
	DOI = {10.3842/SIGMA.2020.097},
	URL = {https://doi.org/10.3842/SIGMA.2020.097},
}


@article {schwedeshipley,
	AUTHOR = {Schwede, Stefan and Shipley, Brooke E.},
	TITLE = {Algebras and modules in monoidal model categories},
	JOURNAL = {Proc. London Math. Soc. (3)},
	FJOURNAL = {Proceedings of the London Mathematical Society. Third Series},
	VOLUME = {80},
	YEAR = {2000},
	NUMBER = {2},
	PAGES = {491--511},
	ISSN = {0024-6115},
	MRCLASS = {18D10 (18D50 55P48 55U35)},
	MRNUMBER = {1734325},
	MRREVIEWER = {Mark Hovey},
	DOI = {10.1112/S002461150001220X},
	URL = {https://doi-org.pros.lib.unimi.it/10.1112/S002461150001220X},
}


@article {aciclicitythm,
	AUTHOR = {Hess, Kathryn and K\c{e}dziorek, Magdalena and Riehl, Emily and
		Shipley, Brooke},
	TITLE = {A necessary and sufficient condition for induced model
		structures},
	JOURNAL = {J. Topol.},
	FJOURNAL = {Journal of Topology},
	VOLUME = {10},
	YEAR = {2017},
	NUMBER = {2},
	PAGES = {324--369},
	ISSN = {1753-8416},
	MRCLASS = {55U35 (18G55)},
	MRNUMBER = {3653314},
	MRREVIEWER = {J\'{e}r\^{o}me Scherer},
	DOI = {10.1112/topo.12011},
	URL = {https://doi-org.pros.lib.unimi.it/10.1112/topo.12011},
}


@article {hovey2,
	AUTHOR = {Hovey, Mark},
	TITLE = {Model category structures on chain complexes of sheaves},
	JOURNAL = {Trans. Amer. Math. Soc.},
	FJOURNAL = {Transactions of the American Mathematical Society},
	VOLUME = {353},
	YEAR = {2001},
	NUMBER = {6},
	PAGES = {2441--2457},
	ISSN = {0002-9947},
	MRCLASS = {18F20 (14F05 18E15 18E30 55U35)},
	MRNUMBER = {1814077},
	MRREVIEWER = {J. F. Jardine},
	DOI = {10.1090/S0002-9947-01-02721-0},
	URL = {https://doi.org/10.1090/S0002-9947-01-02721-0},
}


@article {shipley,
	AUTHOR = {Shipley, Brooke},
	TITLE = {{$H\Bbb Z$}-algebra spectra are differential graded algebras},
	JOURNAL = {Amer. J. Math.},
	FJOURNAL = {American Journal of Mathematics},
	VOLUME = {129},
	YEAR = {2007},
	NUMBER = {2},
	PAGES = {351--379},
	ISSN = {0002-9327},
	MRCLASS = {55P42 (18G55 55P20 55P43 55U35)},
	MRNUMBER = {2306038},
	MRREVIEWER = {Tyler D. Lawson},
	DOI = {10.1353/ajm.2007.0014},
	URL = {https://doi.org/10.1353/ajm.2007.0014},
}


@article {toenchampsaffines,
    AUTHOR = {To\"{e}n, Bertrand},
     TITLE = {Champs affines},
   JOURNAL = {Selecta Math. (N.S.)},
  FJOURNAL = {Selecta Mathematica. New Series},
    VOLUME = {12},
      YEAR = {2006},
    NUMBER = {1},
     PAGES = {39--135},
      ISSN = {1022-1824,1420-9020},
   MRCLASS = {14F35 (14A20 18F10 55U35)},
  MRNUMBER = {2244263},
MRREVIEWER = {Mark\ Hovey},
       DOI = {10.1007/s00029-006-0019-z},
       URL = {https://doi.org/10.1007/s00029-006-0019-z},
}


@book {hovey,
	AUTHOR = {Hovey, Mark},
	TITLE = {Model categories},
	SERIES = {Mathematical Surveys and Monographs},
	VOLUME = {63},
	PUBLISHER = {American Mathematical Society, Providence, RI},
	YEAR = {1999},
	PAGES = {xii+209},
	ISBN = {0-8218-1359-5},
	MRCLASS = {55U35 (18D15 18G30 18G55)},
	MRNUMBER = {1650134},
	MRREVIEWER = {Teimuraz Pirashvili},
}


@misc{pantev2021moduli,
	title={Moduli of flat connections on smooth varieties}, 
	author={Tony Pantev and Bertrand Toën},
	year={2021},
	eprint={1905.12124},
	archivePrefix={arXiv},
	primaryClass={math.AG}
}


@incollection {KSmirrorsymmetry,
	AUTHOR = {Kontsevich, Maxim and Soibelman, Yan},
	TITLE = {Homological mirror symmetry and torus fibrations},
	BOOKTITLE = {Symplectic geometry and mirror symmetry ({S}eoul, 2000)},
	PAGES = {203--263},
	PUBLISHER = {World Sci. Publ., River Edge, NJ},
	YEAR = {2001},
	MRCLASS = {32Q25 (14J32 14K05 18E30 32G05 53C38)},
	MRNUMBER = {1882331},
	MRREVIEWER = {Bal\'{a}zs Szendr\H{o}i},
	DOI = {10.1142/9789812799821_0007},
	URL = {https://doi.org/10.1142/9789812799821_0007},
}


@incollection {beilinsonderived,
    AUTHOR = {Beilinson, A. A.},
     TITLE = {On the derived category of perverse sheaves},
 BOOKTITLE = {{$K$}-theory, arithmetic and geometry ({M}oscow, 1984--1986)},
    SERIES = {Lecture Notes in Math.},
    VOLUME = {1289},
     PAGES = {27--41},
 PUBLISHER = {Springer, Berlin},
      YEAR = {1987},
   MRCLASS = {14F99 (18E30 18F20 32C38 58G07)},
  MRNUMBER = {923133},
MRREVIEWER = {Jean-Luc Brylinski},
       DOI = {10.1007/BFb0078365},
       URL = {https://doi-org.pros.lib.unimi.it:2050/10.1007/BFb0078365},
}
		


@article {beilinsonadic,
	AUTHOR = {Beilinson, A.},
	TITLE = {{$p$}-adic periods and derived de {R}ham cohomology},
	JOURNAL = {J. Amer. Math. Soc.},
	FJOURNAL = {Journal of the American Mathematical Society},
	VOLUME = {25},
	YEAR = {2012},
	NUMBER = {3},
	PAGES = {715--738},
	ISSN = {0894-0347},
	MRCLASS = {14F40 (14F20 14F30 16E45)},
	MRNUMBER = {2904571},
	MRREVIEWER = {Nobuo Tsuzuki},
	DOI = {10.1090/S0894-0347-2012-00729-2},
	URL = {https://doi.org/10.1090/S0894-0347-2012-00729-2},
}




@incollection {lurieelliptic,
	AUTHOR = {Lurie, J.},
	TITLE = {A survey of elliptic cohomology},
	BOOKTITLE = {Algebraic topology},
	SERIES = {Abel Symp.},
	VOLUME = {4},
	PAGES = {219--277},
	PUBLISHER = {Springer, Berlin},
	YEAR = {2009},
	MRCLASS = {55N34 (55P43)},
	MRNUMBER = {2597740},
	MRREVIEWER = {Tyler D. Lawson},
	DOI = {10.1007/978-3-642-01200-6_9},
	URL = {https://doi.org/10.1007/978-3-642-01200-6_9},
}


@book {illusie,
	AUTHOR = {Illusie, Luc},
	TITLE = {Complexe cotangent et d\'{e}formations. {I}},
	SERIES = {Lecture Notes in Mathematics, Vol. 239},
	PUBLISHER = {Springer-Verlag, Berlin-New York},
	YEAR = {1971},
	PAGES = {xv+355},
	MRCLASS = {14B10 (14D15 14F20 55D20)},
	MRNUMBER = {0491680},
	MRREVIEWER = {Larry Breen},
}


@inproceedings {quillenhomology,
	AUTHOR = {Quillen, Daniel},
	TITLE = {On the (co-) homology of commutative rings},
	BOOKTITLE = {Applications of {C}ategorical {A}lgebra ({P}roc. {S}ympos.
		{P}ure {M}ath., {V}ol. {XVII}, {N}ew {Y}ork, 1968)},
	PAGES = {65--87},
	PUBLISHER = {Amer. Math. Soc., Providence, R.I.},
	YEAR = {1970},
	MRCLASS = {13.90 (18.00)},
	MRNUMBER = {0257068},
	MRREVIEWER = {S. Yuan},
}


@article{cohn,
	AUTHOR = {Cohn, Lee},
	TITLE={Differential graded categories are {$k$}-linear stable infinity categories},
	YEAR={2013},
	URL={arXiv:1308.2587},
}


@article {bravdyckerhoff2,
	AUTHOR = {Brav, Christopher and Dyckerhoff, Tobias},
	TITLE = {Relative {C}alabi-{Y}au structures {II}: shifted {L}agrangians
		in the moduli of objects},
	JOURNAL = {Selecta Math. (N.S.)},
	FJOURNAL = {Selecta Mathematica. New Series},
	VOLUME = {27},
	YEAR = {2021},
	NUMBER = {4},
	PAGES = {Paper No. 63, 45},
	ISSN = {1022-1824},
	MRCLASS = {14F08 (14D23 14J32 18G35 18G80 53C55)},
	MRNUMBER = {4281260},
	MRREVIEWER = {\Dbar \cftil{o} Ng\d{o}c Di\cfudot{e}p},
	DOI = {10.1007/s00029-021-00642-5},
	URL = {https://doi.org/10.1007/s00029-021-00642-5},
}




@book {loday,
	AUTHOR = {Loday, Jean-Louis},
	TITLE = {Cyclic homology},
	SERIES = {Grundlehren der Mathematischen Wissenschaften [Fundamental
		Principles of Mathematical Sciences]},
	VOLUME = {301},
	EDITION = {Second},
	NOTE = {Appendix E by Mar\'{\i}a O. Ronco,
		Chapter 13 by the author in collaboration with Teimuraz
		Pirashvili},
	PUBLISHER = {Springer-Verlag, Berlin},
	YEAR = {1998},
	PAGES = {xx+513},
	ISBN = {3-540-63074-0},
	MRCLASS = {16E40 (13D03 17B55 18G60 19D55)},
	MRNUMBER = {1600246},
	DOI = {10.1007/978-3-662-11389-9},
	URL = {https://doi.org/10.1007/978-3-662-11389-9},
}


@article {BGT,
	AUTHOR = {Blumberg, Andrew J. and Gepner, David and Tabuada, Gon\c{c}alo},
	TITLE = {A universal characterization of higher algebraic {$K$}-theory},
	JOURNAL = {Geom. Topol.},
	FJOURNAL = {Geometry \& Topology},
	VOLUME = {17},
	YEAR = {2013},
	NUMBER = {2},
	PAGES = {733--838},
	ISSN = {1465-3060},
	MRCLASS = {19D10 (18D20 19D25 19D55 55N15 55U40)},
	MRNUMBER = {3070515},
	MRREVIEWER = {Ross Staffeldt},
	DOI = {10.2140/gt.2013.17.733},
	URL = {https://doi.org/10.2140/gt.2013.17.733},
}


@article {cyclichomology2,
	AUTHOR = {Keller, Bernhard},
	TITLE = {On the cyclic homology of ringed spaces and schemes},
	JOURNAL = {Doc. Math.},
	FJOURNAL = {Documenta Mathematica},
	VOLUME = {3},
	YEAR = {1998},
	PAGES = {231--259},
	ISSN = {1431-0635},
	MRCLASS = {16E40 (14F05 18E30)},
	MRNUMBER = {1647519},
	MRREVIEWER = {Kevin P. Knudson},
}


@article {orlov,
	AUTHOR = {Orlov, Dmitri},
	TITLE = {Smooth and proper noncommutative schemes and gluing of {DG}
		categories},
	JOURNAL = {Adv. Math.},
	FJOURNAL = {Advances in Mathematics},
	VOLUME = {302},
	YEAR = {2016},
	PAGES = {59--105},
	ISSN = {0001-8708},
	MRCLASS = {14F05 (16E45 18E30)},
	MRNUMBER = {3545926},
	MRREVIEWER = {Shintarou Yanagida},
	DOI = {10.1016/j.aim.2016.07.014},
	URL = {https://doi.org/10.1016/j.aim.2016.07.014},
}


@article {keller2,
	AUTHOR = {Keller, Bernhard},
	TITLE = {Deriving {DG} categories},
	JOURNAL = {Ann. Sci. \'{E}cole Norm. Sup. (4)},
	FJOURNAL = {Annales Scientifiques de l'\'{E}cole Normale Sup\'{e}rieure. Quatri\`eme
		S\'{e}rie},
	VOLUME = {27},
	YEAR = {1994},
	NUMBER = {1},
	PAGES = {63--102},
	ISSN = {0012-9593},
	MRCLASS = {18E30 (16D90)},
	MRNUMBER = {1258406},
	MRREVIEWER = {Jeremy Rickard},
	URL = {http://www.numdam.org/item?id=ASENS_1994_4_27_1_63_0},
}


@article {hag1,
	AUTHOR = {To\"{e}n, Bertrand and Vezzosi, Gabriele},
	TITLE = {Homotopical algebraic geometry. {I}. {T}opos theory},
	JOURNAL = {Adv. Math.},
	FJOURNAL = {Advances in Mathematics},
	VOLUME = {193},
	YEAR = {2005},
	NUMBER = {2},
	PAGES = {257--372},
	ISSN = {0001-8708},
	MRCLASS = {14F20 (18F20 18G55 55U40)},
	MRNUMBER = {2137288},
	MRREVIEWER = {Paul Arne \O stv\ae r},
	DOI = {10.1016/j.aim.2004.05.004},
	URL = {https://doi.org/10.1016/j.aim.2004.05.004},
}


@article {hag2,
	AUTHOR = {To\"{e}n, Bertrand and Vezzosi, Gabriele},
	TITLE = {Homotopical algebraic geometry. {II}. {G}eometric stacks and
		applications},
	JOURNAL = {Mem. Amer. Math. Soc.},
	FJOURNAL = {Memoirs of the American Mathematical Society},
	VOLUME = {193},
	YEAR = {2008},
	NUMBER = {902},
	PAGES = {x+224},
	ISSN = {0065-9266},
	MRCLASS = {14A20 (18F10 18F20 18G55 55P42 55U40)},
	MRNUMBER = {2394633},
	MRREVIEWER = {Paul Arne \O stv\ae r},
	DOI = {10.1090/memo/0902},
	URL = {https://doi.org/10.1090/memo/0902},
}


@article{BCS,
	AUTHOR={Bozec, Tristan and Calaque, Damien and Scherotzke, Sarah},
	TITLE={Relative critical loci and quiver moduli},
	YEAR={2021},
	URL = {arXiv:2006.01069v2},
}


@article{robalo,
	AUTHOR={Robalo, Marco},
	TITLE={Noncommutative Motives I: A Universal Characterization of the Motivic Stable Homotopy Theory of Schemes},
	YEAR={2013},
	URL = {arXiv:1206.3645v3},
}


@article {keller,
	AUTHOR = {Keller, Bernhard},
	TITLE = {On the cyclic homology of exact categories},
	JOURNAL = {J. Pure Appl. Algebra},
	FJOURNAL = {Journal of Pure and Applied Algebra},
	VOLUME = {136},
	YEAR = {1999},
	NUMBER = {1},
	PAGES = {1--56},
	ISSN = {0022-4049},
	MRCLASS = {18G60 (18E10)},
	MRNUMBER = {1667558},
	MRREVIEWER = {Teimuraz Pirashvili},
	DOI = {10.1016/S0022-4049(97)00152-7},
	URL = {https://doi.org/10.1016/S0022-4049(97)00152-7},
}


@article {iteratedspans,
	AUTHOR = {Haugseng, Rune},
	TITLE = {Iterated spans and classical topological field theories},
	JOURNAL = {Math. Z.},
	FJOURNAL = {Mathematische Zeitschrift},
	VOLUME = {289},
	YEAR = {2018},
	NUMBER = {3-4},
	PAGES = {1427--1488},
	ISSN = {0025-5874},
	MRCLASS = {18D05 (14A20 14F05 81R10)},
	MRNUMBER = {3830256},
	DOI = {10.1007/s00209-017-2005-x},
	URL = {https://doi.org/10.1007/s00209-017-2005-x},
}


@article {igusa,
	AUTHOR = {Igusa, Jun-ichi},
	TITLE = {Fibre systems of {J}acobian varieties. {III}. {F}ibre systems
		of elliptic curves},
	JOURNAL = {Amer. J. Math.},
	FJOURNAL = {American Journal of Mathematics},
	VOLUME = {81},
	YEAR = {1959},
	PAGES = {453--476},
	ISSN = {0002-9327},
	MRCLASS = {14.00},
	MRNUMBER = {0104669},
	MRREVIEWER = {M. Rosenlicht},
	DOI = {10.2307/2372751},
	URL = {https://doi.org/10.2307/2372751},
}


@article {drinfeld,
	AUTHOR = {Drinfeld, V. G.},
	TITLE = {Elliptic modules},
	JOURNAL = {Mat. Sb. (N.S.)},
	VOLUME = {94(136)},
	YEAR = {1974},
	PAGES = {594--627, 656},
	MRCLASS = {10D99 (14K15)},
	MRNUMBER = {0384707},
	MRREVIEWER = {Pierre Deligne},
}


@article {DR,
	AUTHOR = {Deligne, P. and Rapoport, M.},
	TITLE = {Les sch\'{e}mas de modules de courbes elliptiques},
	BOOKTITLE = {Modular functions of one variable, {II} ({P}roc. {I}nternat.
		{S}ummer {S}chool, {U}niv. {A}ntwerp, {A}ntwerp, 1972)},
	PAGES = {143--316. Lecture Notes in Math., Vol. 349},
	PUBLISHER = {Springer, Berlin},
	YEAR = {1973},
	MRCLASS = {14K10 (10D05)},
	MRNUMBER = {0337993},
	MRREVIEWER = {T. Oda},
}


@book {KM,
	AUTHOR = {Katz, Nicholas M. and Mazur, Barry},
	TITLE = {Arithmetic moduli of elliptic curves},
	SERIES = {Annals of Mathematics Studies},
	VOLUME = {108},
	PUBLISHER = {Princeton University Press, Princeton, NJ},
	YEAR = {1985},
	PAGES = {xiv+514},
	ISBN = {0-691-08349-5; 0-691-08352-5},
	MRCLASS = {11G05 (11F11 14G25 14K15)},
	MRNUMBER = {772569},
	MRREVIEWER = {Kenneth A. Ribet},
	DOI = {10.1515/9781400881710},
	URL = {https://doi.org/10.1515/9781400881710},
}


@article{CPTVV,
	AUTHOR = {Calaque, Damien and Pantev, Tony and To\"{e}n, Bertrand and
		Vaqui\'{e}, Michel and Vezzosi, Gabriele},
	TITLE = {Shifted {P}oisson structures and deformation quantization},
	JOURNAL = {J. Topol.},
	FJOURNAL = {Journal of Topology},
	VOLUME = {10},
	YEAR = {2017},
	NUMBER = {2},
	PAGES = {483--584},
	ISSN = {1753-8416},
	MRCLASS = {14A20 (14D15 14F05 18E30 18G55 53D55)},
	MRNUMBER = {3653319},
	MRREVIEWER = {Scott R. Nollet},
	DOI = {10.1112/topo.12012},
	URL = {https://doi.org/10.1112/topo.12012},
}

@book{1,
	author = {Mobilio, Settimio and Boscherini, Federico and Meneghini, C.},
	year = {2015},
	month = {01},
	pages = {1-799},
	title = {Synchrotron radiation: Basics, methods and applications},
	doi = {10.1007/978-3-642-55315-8}
}


@Misc{2,
	AUTHOR = {Barbarino, Sebastiano},
	TITLE = {Appunti di Campi Elettromagnetici},
	YEAR = {2013},
	URL = {http://www.diit.unict.it/users/campi/appunti_campi_indice.htm},
}


@misc{calaque2021lie,
	title={Lie algebroids are curved Lie algebras}, 
	author={Damien Calaque and Ricardo Campos and Joost Nuiten},
	year={2021},
	eprint={2103.10728},
	archivePrefix={arXiv},
	primaryClass={math.AT}
}


@article {PTVV,
AUTHOR = {Pantev, Tony and To\"{e}n, Bertrand and Vaqui\'{e}, Michel and
	Vezzosi, Gabriele},
TITLE = {Shifted symplectic structures},
JOURNAL = {Publ. Math. Inst. Hautes \'{E}tudes Sci.},
FJOURNAL = {Publications Math\'{e}matiques. Institut de Hautes \'{E}tudes
	Scientifiques},
VOLUME = {117},
YEAR = {2013},
PAGES = {271--328},
ISSN = {0073-8301},
MRCLASS = {14F05 (14A15 18F20 18G30 53D05 53D12)},
MRNUMBER = {3090262},
MRREVIEWER = {Andrey Yu. Lazarev},
DOI = {10.1007/s10240-013-0054-1},
URL = {https://doi.org/10.1007/s10240-013-0054-1},
}


@article {sullivanmodel,
    AUTHOR = {Sullivan, Dennis},
     TITLE = {Infinitesimal computations in topology},
   JOURNAL = {Inst. Hautes \'{E}tudes Sci. Publ. Math.},
  FJOURNAL = {Institut des Hautes \'{E}tudes Scientifiques. Publications
              Math\'{e}matiques},
    NUMBER = {47},
      YEAR = {1977},
     PAGES = {269--331},
      ISSN = {0073-8301,1618-1913},
   MRCLASS = {57D99 (55D99 58A10)},
  MRNUMBER = {646078},
MRREVIEWER = {J.\ F.\ Adams},
       URL = {http://www.numdam.org/item?id=PMIHES_1977__47__269_0},
}


@article {plderham,
    AUTHOR = {Bousfield, A. K. and Gugenheim, V. K. A. M.},
     TITLE = {On {${\rm PL}$} de {R}ham theory and rational homotopy type},
   JOURNAL = {Mem. Amer. Math. Soc.},
  FJOURNAL = {Memoirs of the American Mathematical Society},
    VOLUME = {8},
      YEAR = {1976},
    NUMBER = {179},
     PAGES = {ix+94},
      ISSN = {0065-9266,1947-6221},
   MRCLASS = {55D15 (58A10)},
  MRNUMBER = {425956},
MRREVIEWER = {Jean-Michel\ Lemaire},
       DOI = {10.1090/memo/0179},
       URL = {https://doi.org/10.1090/memo/0179},
}


@article {berglundkoszul,
    AUTHOR = {Berglund, Alexander},
     TITLE = {Koszul spaces},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {366},
      YEAR = {2014},
    NUMBER = {9},
     PAGES = {4551--4569},
      ISSN = {0002-9947,1088-6850},
   MRCLASS = {55P62 (16S37 18D50)},
  MRNUMBER = {3217692},
MRREVIEWER = {Samuel\ B.\ Smith},
       DOI = {10.1090/S0002-9947-2014-05935-7},
       URL = {https://doi.org/10.1090/S0002-9947-2014-05935-7},
}


@book {studyindag2,
	AUTHOR = {Gaitsgory, Dennis and Rozenblyum, Nick},
	TITLE = {A study in derived algebraic geometry. {V}ol. {II}.
		{D}eformations, {L}ie theory and formal geometry},
	SERIES = {Mathematical Surveys and Monographs},
	VOLUME = {221},
	PUBLISHER = {American Mathematical Society, Providence, RI},
	YEAR = {2017},
	PAGES = {xxxv+436},
	ISBN = {978-1-4704-3570-7},
	MRCLASS = {14F05 (18D05 18G55)},
	MRNUMBER = {3701353},
	MRREVIEWER = {Adrian Langer},
	DOI = {10.1090/surv/221.2},
	URL = {https://doi.org/10.1090/surv/221.2},
}


@book {studyindag1,
	AUTHOR = {Gaitsgory, Dennis and Rozenblyum, Nick},
	TITLE = {A study in derived algebraic geometry. {V}ol. {I}.
		{C}orrespondences and duality},
	SERIES = {Mathematical Surveys and Monographs},
	VOLUME = {221},
	PUBLISHER = {American Mathematical Society, Providence, RI},
	YEAR = {2017},
	PAGES = {xl+533pp},
	ISBN = {978-1-4704-3569-1},
	MRCLASS = {14F05 (18D05 18G55)},
	MRNUMBER = {3701352},
	MRREVIEWER = {Adrian Langer},
	DOI = {10.1090/surv/221.1},
	URL = {https://doi.org/10.1090/surv/221.1},
}


@book {weibel,
	AUTHOR = {Weibel, Charles A.},
	TITLE = {An introduction to homological algebra},
	SERIES = {Cambridge Studies in Advanced Mathematics},
	VOLUME = {38},
	PUBLISHER = {Cambridge University Press, Cambridge},
	YEAR = {1994},
	PAGES = {xiv+450},
	ISBN = {0-521-43500-5; 0-521-55987-1},
	MRCLASS = {18-01 (16-01 17-01 20-01 55Uxx)},
	MRNUMBER = {1269324},
	MRREVIEWER = {Kenneth A. Brown},
	DOI = {10.1017/CBO9781139644136},
	URL = {https://doi-org.pros.lib.unimi.it/10.1017/CBO9781139644136},
}


@Book{weil,
title      = {Introduction \`a l'\'etude des vari\'et\'es k\"ahl\'eriennes},
publisher  = {Hermann, Paris},
year       = {1958},
author     = {Weil, Andr\'e},
series     = {Publications de l'Institut de Math\'ematique de l'Universit\'e de Nancago, VI. Actualit\'es Sci. Ind. no. 1267},
mrclass    = {57.00},
mrnumber   = {0111056},
mrreviewer = {F. Hirzebruch},
pages      = {175},
}


@book {rosicky,
	AUTHOR = {Ad\'{a}mek, Ji\v{r}\'{\i} and Rosick\'{y}, Ji\v{r}\'{\i}},
	TITLE = {Locally presentable and accessible categories},
	SERIES = {London Mathematical Society Lecture Note Series},
	VOLUME = {189},
	PUBLISHER = {Cambridge University Press, Cambridge},
	YEAR = {1994},
	PAGES = {xiv+316},
	ISBN = {0-521-42261-2},
	MRCLASS = {18Axx (18-02)},
	MRNUMBER = {1294136},
	MRREVIEWER = {J. R. Isbell},
	DOI = {10.1017/CBO9780511600579},
	URL = {https://doi.org/10.1017/CBO9780511600579},
}


@Book{htt,
AUTHOR = {Lurie, Jacob},
TITLE = {Higher topos theory},
SERIES = {Annals of Mathematics Studies},
VOLUME = {170},
PUBLISHER = {Princeton University Press, Princeton, NJ},
YEAR = {2009},
PAGES = {xviii+925},
ISBN = {978-0-691-14049-0},
MRCLASS = {18-02 (18B25 18E35 18G30 18G55 55U40)},
MRNUMBER = {2522659},
MRREVIEWER = {Mark Hovey},
DOI = {10.1515/9781400830558},
URL = {https://doi.org/10.1515/9781400830558},
}


@article {tstructurektheory,
	AUTHOR = {Antieau, Benjamin and Gepner, David and Heller, Jeremiah},
	TITLE = {{$K$}-theoretic obstructions to bounded {$t$}-structures},
	JOURNAL = {Invent. Math.},
	FJOURNAL = {Inventiones Mathematicae},
	VOLUME = {216},
	YEAR = {2019},
	NUMBER = {1},
	PAGES = {241--300},
	ISSN = {0020-9910},
	MRCLASS = {19D35 (16E45 16P40 18E10 18E30 55P43)},
	MRNUMBER = {3935042},
	MRREVIEWER = {Guillermo Corti\~{n}as},
	DOI = {10.1007/s00222-018-00847-0},
	URL = {https://doi-org.pros2.lib.unimi.it/10.1007/s00222-018-00847-0},
}


@article {gepnerhaugseng,
    AUTHOR = {Gepner, David and Haugseng, Rune},
     TITLE = {Enriched {$\infty$}-categories via non-symmetric
              {$\infty$}-operads},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {279},
      YEAR = {2015},
     PAGES = {575--716},
      ISSN = {0001-8708},
   MRCLASS = {18D20 (18D10 18D50)},
  MRNUMBER = {3345192},
MRREVIEWER = {Christopher L. Rogers},
       DOI = {10.1016/j.aim.2015.02.007},
       URL = {https://doi.org/10.1016/j.aim.2015.02.007},
}


@Misc{HA,
AUTHOR = {Lurie, Jacob},
TITLE = {Higher Algebra},
YEAR = {2017},
PAGES = {1553},
URL = {http://www.math.harvard.edu/~lurie/papers/HA.pdf},
}


@Misc{portasala,
AUTHOR = {Porta, Mauro and Sala, Francesco},
TITLE = {Simpson’s shapes of schemes and stacks},
YEAR = {2020},
URL = {https://people.dm.unipi.it/sala/assets/pdf/porta_sala_shapes.pdf},
}

@misc{carmeli2023characterstransfermapscategorified,
      title={Characters and transfer maps via categorified traces}, 
      author={Shachar Carmeli and Bastiaan Cnossen and Maxime Ramzi and Lior Yanovski},
      year={2023},
      eprint={2210.17364},
      archivePrefix={arXiv},
      primaryClass={math.AT},
      url={https://arxiv.org/abs/2210.17364}, 
}

@misc{benmoshe2024categoricalambidexterity,
      title={Categorical Ambidexterity}, 
      author={Shay Ben-Moshe},
      year={2024},
      eprint={2411.17281},
      archivePrefix={arXiv},
      primaryClass={math.CT},
      url={https://arxiv.org/abs/2411.17281}, 
}


@misc{mazelgee2021universal,
      title={A universal characterization of noncommutative motives and secondary algebraic K-theory}, 
      author={Aaron Mazel-Gee and Reuben Stern},
      year={2021},
      eprint={2104.04021},
      archivePrefix={arXiv},
      primaryClass={math.KT}
}


@article{pare, title={Simply Connected Limits}, volume={42}, DOI={10.4153/CJM-1990-038-6}, number={4}, journal={Canadian Journal of Mathematics}, publisher={Cambridge University Press}, author={Paré, Robert}, year={1990}, pages={731–746}}


@Misc{sag,
	AUTHOR = {Lurie, Jacob},
	TITLE = {Spectral Algebraic Geometry (Under Construction)},
	YEAR = {2018},
	URL = {https://www.math.ias.edu/~lurie/papers/SAG-rootfile.pdf},
}


@article{heineenrichedaction,
title = {An equivalence between enriched $\infty$-categories and $\infty$-categories with weak action},
journal = {Advances in Mathematics},
volume = {417},
pages = {108941},
year = {2023},
issn = {0001-8708},
doi = {https://doi.org/10.1016/j.aim.2023.108941},
url = {https://www.sciencedirect.com/science/article/pii/S0001870823000841},
author = {Hadrian Heine},
}


@misc{schreiber2013differential,
      title={Differential cohomology in a cohesive infinity-topos}, 
      author={Urs Schreiber},
      year={2013},
      eprint={1310.7930},
      archivePrefix={arXiv},
      primaryClass={math-ph}
}


@article {holstein,
    AUTHOR = {Holstein, Julian V. S.},
     TITLE = {Morita cohomology and homotopy locally constant sheaves},
   JOURNAL = {Math. Proc. Cambridge Philos. Soc.},
  FJOURNAL = {Mathematical Proceedings of the Cambridge Philosophical
              Society},
    VOLUME = {158},
      YEAR = {2015},
    NUMBER = {1},
     PAGES = {27--35},
      ISSN = {0305-0041,1469-8064},
   MRCLASS = {55N30 (18G60)},
  MRNUMBER = {3300313},
MRREVIEWER = {Timothy\ Porter},
       DOI = {10.1017/S0305004114000528},
       URL = {https://doi.org/10.1017/S0305004114000528},
}


@book {sadun,
    AUTHOR = {Sadun, Lorenzo},
     TITLE = {Topology of tiling spaces},
    SERIES = {University Lecture Series},
    VOLUME = {46},
 PUBLISHER = {American Mathematical Society, Providence, RI},
      YEAR = {2008},
     PAGES = {x+118},
      ISBN = {978-0-8218-4727-5},
   MRCLASS = {52C22 (37B50 52C23 55N05)},
  MRNUMBER = {2446623},
MRREVIEWER = {Bernd\ Sing},
       DOI = {10.1090/ulect/046},
       URL = {https://doi.org/10.1090/ulect/046},
}


@Misc{dagviii,
	AUTHOR = {Lurie, Jacob},
	TITLE = {Derived Algebraic Geometry VIII: Quasi-Coherent Sheaves and
		Tannaka Duality Theorems},
	YEAR = {2011},
	URL = {http://people.math.harvard.edu/~lurie/papers/DAG-VIII.pdf},
}


@Misc{dagvii,
	AUTHOR = {Lurie, Jacob},
	TITLE = {Derived Algebraic Geometry VII: Spectral Schemes},
	YEAR = {2011},
	URL = {https://people.math.harvard.edu/~lurie/papers/DAG-VII.pdf},
}


@Misc{dagx,
	AUTHOR = {Lurie, Jacob},
	TITLE = {Derived Algebraic Geometry X: Formal Moduli Problems},
	YEAR = {2011},
	URL = {http://people.math.harvard.edu/~lurie/papers/DAG-X.pdf},
}

@Misc{dagxiii,
	AUTHOR = {Lurie, Jacob},
	TITLE = {Derived Algebraic Geometry XIII: Rational and $p$-adic Homotopy Theory},
	YEAR = {2011},
	URL = {http://people.math.harvard.edu/~lurie/papers/DAG-XIII.pdf},
}



@Misc{ellipticcohomology1,
	AUTHOR = {Lurie, Jacob},
	TITLE = {Elliptic Cohomology I: Spectral Abelian Varieties},
	YEAR = {2018},
	URL = {http://people.math.harvard.edu/~lurie/papers/Elliptic-I.pdf},
}


@Misc{schwedespectra,
	AUTHOR = {Schwede, Stefan},
	TITLE = {Symmetric Spectra},
	YEAR = {2012},
	URL = {http://www.math.uni-bonn.de/people/schwede/SymSpec-v3.pdf},
}


@article {bravdyckerhoff,
AUTHOR = {Brav, Christopher and Dyckerhoff, Tobias},
TITLE = {Relative {C}alabi-{Y}au structures},
JOURNAL = {Compos. Math.},
FJOURNAL = {Compositio Mathematica},
VOLUME = {155},
YEAR = {2019},
NUMBER = {2},
PAGES = {372--412},
ISSN = {0010-437X},
MRCLASS = {18E30 (14F05 32Q25 58B34)},
MRNUMBER = {3911626},
DOI = {10.1112/s0010437x19007024},
URL = {https://doi.org/10.1112/s0010437x19007024},
}


@article {toenvaquie,
AUTHOR = {To\"{e}n, Bertrand and Vaqui\'{e}, Michel},
TITLE = {Moduli of objects in dg-categories},
JOURNAL = {Ann. Sci. \'{E}cole Norm. Sup. (4)},
FJOURNAL = {Annales Scientifiques de l'\'{E}cole Normale Sup\'{e}rieure. Quatri\`eme
	S\'{e}rie},
VOLUME = {40},
YEAR = {2007},
NUMBER = {3},
PAGES = {387--444},
ISSN = {0012-9593},
MRCLASS = {18G55 (14D20 18E30)},
MRNUMBER = {2493386},
MRREVIEWER = {Andrey Yu. Lazarev},
DOI = {10.1016/j.ansens.2007.05.001},
URL = {https://doi.org/10.1016/j.ansens.2007.05.001},
}


@article {verdier,
AUTHOR = {Verdier, Jean-Louis},
TITLE = {Des cat\'{e}gories d\'{e}riv\'{e}es des cat\'{e}gories ab\'{e}liennes},
NOTE = {With a preface by Luc Illusie,
	Edited and with a note by Georges Maltsiniotis},
JOURNAL = {Ast\'{e}risque},
FJOURNAL = {Ast\'{e}risque},
NUMBER = {239},
YEAR = {1996},
PAGES = {xii+253 pp. (1997)},
ISSN = {0303-1179},
MRCLASS = {18E30 (18-03 18E35)},
MRNUMBER = {1453167},
MRREVIEWER = {Amnon Neeman},
}




@Article{vialekahn,
author   = {Barbieri-Viale, Luca and Kahn, Bruno},
title    = {On the derived category of 1-motives},
journal  = {Ast\'erisque},
year     = {2016},
number   = {381},
pages    = {xi+254},
issn     = {0303-1179},
fjournal = {Ast\'erisque},
isbn     = {978-2-85629-837-4},
mrclass  = {14F05 (14C30 14F20 18E30)},
mrnumber = {3545132},
}


@Article{vialesrinivas,
author     = {Barbieri-Viale, Luca and Srinivas, Vasudevan},
title      = {Albanese and {P}icard 1-motives},
journal    = {M\'em. Soc. Math. Fr. (N.S.)},
year       = {2001},
number     = {87},
pages      = {vi+104},
issn       = {0249-633X},
fjournal   = {M\'emoires de la Soci\'et\'e Math\'ematique de France. Nouvelle S\'erie},
mrclass    = {14C30 (14F42 14K30)},
mrnumber   = {1891270},
mrreviewer = {Tam\~A!`s Szamuely},
}


@misc{GPS,
    title={Mirror symmetry: from categories to curve counts},
    author={Sheel Ganatra and Timothy Perutz and Nick Sheridan},
    year={2015},
    eprint={1510.03839},
    archivePrefix={arXiv},
    primaryClass={math.SG}
}


@Article{HMS,
author={Haugseng, Rune, and Melani, Valerio and Safronov, Pavel},
title={Shifted coisotropic correspondences},
year={2019},
url={	arXiv:1904.11312},
}


@Article{barbierisaito,
author     = {Barbieri-Viale, L. and Rosenschon, A. and Saito, M.},
title      = {Deligne's conjecture on 1-motives},
journal    = {Ann. of Math. (2)},
year       = {2003},
volume     = {158},
number     = {2},
pages      = {593--633},
issn       = {0003-486X},
doi        = {10.4007/annals.2003.158.593},
fjournal   = {Annals of Mathematics. Second Series},
mrclass    = {14C30 (14D07)},
mrnumber   = {2018930},
mrreviewer = {H\~A\copyright{}l\~A\"{\ }ne Esnault},
url        = {http://dx.doi.org/10.4007/annals.2003.158.593},
}


@Book{berthelot,
title      = {Th\'eorie de {D}ieudonn\'e cristalline. {II}},
publisher  = {Springer-Verlag, Berlin},
year       = {1982},
author     = {Berthelot, Pierre and Breen, Lawrence and Messing, William},
volume     = {930},
series     = {Lecture Notes in Mathematics},
isbn       = {3-540-11556-0},
doi        = {10.1007/BFb0093025},
mrclass    = {14L05 (14F30)},
mrnumber   = {667344},
mrreviewer = {Lucile B\~A\copyright{}gueri},
pages      = {x+261},
url        = {http://dx.doi.org/10.1007/BFb0093025},
}

@book {Bosch_rigid_geometry,
    AUTHOR = {Bosch, Siegfried},
     TITLE = {Lectures on formal and rigid geometry},
    SERIES = {Lecture Notes in Mathematics},
    VOLUME = {2105},
 PUBLISHER = {Springer, Cham},
      YEAR = {2014},
     PAGES = {viii+254},
      ISBN = {978-3-319-04416-3; 978-3-319-04417-0},
   MRCLASS = {14G22 (11S85 14-02 14D15)},
  MRNUMBER = {3309387},
MRREVIEWER = {Alessandra\ Bertapelle},
       DOI = {10.1007/978-3-319-04417-0},
       URL = {https://doi.org/10.1007/978-3-319-04417-0},
}


@Book{neronmodels,
title      = {N\'eron models},
publisher  = {Springer-Verlag, Berlin},
year       = {1990},
author     = {Bosch, Siegfried and L\"utkebohmert, Werner and Raynaud, Michel},
volume     = {21},
series     = {Ergebnisse der Mathematik und ihrer Grenzgebiete (3) [Results in Mathematics and Related Areas (3)]},
isbn       = {3-540-50587-3},
doi        = {10.1007/978-3-642-51438-8},
mrclass    = {14K15 (11G10 14L15)},
mrnumber   = {1045822},
mrreviewer = {James Milne},
pages      = {x+325},
url        = {http://dx.doi.org/10.1007/978-3-642-51438-8},
}


@Misc{mixedmotives,
author       = {Cisinski, Denis-Charles and Déglise, Frédéric},
title        = {Triangulated categories of mixed motives},
howpublished = {https://arxiv.org/pdf/0912.2110.pdf},
month        = {Dec},
year         = {2012},
publisher    = {arXiv:0912.2110v3},
}


@Article{delignelefschetz,
author     = {Deligne, P.},
title      = {Th\'eor\`eme de {L}efschetz et crit\`eres de d\'eg\'en\'erescence de suites spectrales},
journal    = {Inst. Hautes \'Etudes Sci. Publ. Math.},
year       = {1968},
number     = {35},
pages      = {259--278},
issn       = {0073-8301},
fjournal   = {Institut des Hautes \'Etudes Scientifiques. Publications Math\'ematiques},
mrclass    = {14.52},
mrnumber   = {0244265},
mrreviewer = {D. I. Lieberman},
url        = {http://www.numdam.org/item?id=PMIHES_1968__35__259_0},
}


@Article{hodgetheory2,
author     = {Deligne, Pierre},
title      = {Th\'eorie de {H}odge. {II}},
journal    = {Inst. Hautes \'Etudes Sci. Publ. Math.},
year       = {1971},
number     = {40},
pages      = {5--57},
issn       = {0073-8301},
fjournal   = {Institut des Hautes \'Etudes Scientifiques. Publications Math\'ematiques},
mrclass    = {14C30 (14F15)},
mrnumber   = {0498551},
mrreviewer = {J. H. M. Steenbrink},
url        = {http://www.numdam.org/item?id=PMIHES_1971__40__5_0},
}


@Article{hodgetheory3,
author     = {Deligne, Pierre},
title      = {Th\'eorie de {H}odge. {III}},
journal    = {Inst. Hautes \'Etudes Sci. Publ. Math.},
year       = {1974},
number     = {44},
pages      = {5--77},
issn       = {0073-8301},
fjournal   = {Institut des Hautes \'Etudes Scientifiques. Publications Math\'ematiques},
mrclass    = {14C30 (14F15)},
mrnumber   = {0498551},
mrreviewer = {J. H. M. Steenbrink},
url        = {http://www.numdam.org/item?id=PMIHES_1971__40__5_0},
}


@Misc{moonen,
author       = {Moonen, Ben and van der Geer, Gerard and Edixhoven, Bas},
title        = {Abelian Varieties},
howpublished = {http://www.mi.fu-berlin.de/users/elenalavanda/BMoonen.pdf},
note         = {Preliminary version},
}


@incollection {lipmanadjointassociativity,
	AUTHOR = {Lipman, Joseph},
	TITLE = {Adjoint associativity: an invitation to algebra in
		{$\infty$}-categories},
	BOOKTITLE = {Commutative algebra and noncommutative algebraic geometry.
		{V}ol. {II}},
	SERIES = {Math. Sci. Res. Inst. Publ.},
	VOLUME = {68},
	PAGES = {265--291},
	PUBLISHER = {Cambridge Univ. Press, New York},
	YEAR = {2015},
	MRCLASS = {14F05 (13D03 13D09 18D10 18D35 18G55)},
	MRNUMBER = {3496871},
	MRREVIEWER = {\Dbar \cftil{o} Ng\d{o}c Di\cfudot{e}p},
}

@book {MR0241495,
    AUTHOR = {Grothendieck, A.},
     TITLE = {Cat\'{e}gories cofibr\'{e}es additives et complexe cotangent
              relatif},
    SERIES = {Lecture Notes in Mathematics},
    VOLUME = {No. 79},
 PUBLISHER = {Springer-Verlag, Berlin-New York},
      YEAR = {1968},
     PAGES = {ii+167},
   MRCLASS = {18.10 (14.00)},
  MRNUMBER = {241495},
MRREVIEWER = {P.\ Abellanas},
}

@book {complexcotangent2,
	AUTHOR = {Illusie, Luc},
	TITLE = {Complexe cotangent et d\'{e}formations. {II}},
	SERIES = {Lecture Notes in Mathematics, Vol. 283},
	PUBLISHER = {Springer-Verlag, Berlin-New York},
	YEAR = {1972},
	PAGES = {vii+304},
	MRCLASS = {14B10 (14D15 14F20 55D20)},
	MRNUMBER = {0491681},
	MRREVIEWER = {Larry Breen},
}

@book {MR0146040,
    AUTHOR = {Grothendieck, Alexander},
     TITLE = {Fondements de la g\'{e}om\'{e}trie alg\'{e}brique. [{E}xtraits
              du {S}\'{e}minaire {B}ourbaki, 1957--1962.]},
 PUBLISHER = {Secr\'{e}tariat math\'{e}matique, Paris},
      YEAR = {1962},
     PAGES = {ii+205},
   MRCLASS = {14.00},
  MRNUMBER = {146040},
}

@article {MR0217093,
    AUTHOR = {Schlessinger, Michael},
     TITLE = {Functors of {A}rtin rings},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {130},
      YEAR = {1968},
     PAGES = {208--222},
      ISSN = {0002-9947,1088-6850},
   MRCLASS = {14.55},
  MRNUMBER = {217093},
MRREVIEWER = {M.\ Miyanishi},
       DOI = {10.2307/1994967},
       URL = {https://doi.org/10.2307/1994967},
}

@book {MR0815922,
    AUTHOR = {Kodaira, Kunihiko},
     TITLE = {Complex manifolds and deformation of complex structures},
    SERIES = {Grundlehren der mathematischen Wissenschaften [Fundamental
              Principles of Mathematical Sciences]},
    VOLUME = {283},
      NOTE = {Translated from the Japanese by Kazuo Akao,
              With an appendix by Daisuke Fujiwara},
 PUBLISHER = {Springer-Verlag, New York},
      YEAR = {1986},
     PAGES = {x+465},
      ISBN = {0-387-96188-7},
   MRCLASS = {32G05 (32-02)},
  MRNUMBER = {815922},
MRREVIEWER = {James\ A.\ Carlson},
       DOI = {10.1007/978-1-4613-8590-5},
       URL = {https://doi.org/10.1007/978-1-4613-8590-5},
}

@article {MR0195995,
    AUTHOR = {Nijenhuis, Albert and Richardson, Jr., R. W.},
     TITLE = {Cohomology and deformations in graded {L}ie algebras},
   JOURNAL = {Bull. Amer. Math. Soc.},
  FJOURNAL = {Bulletin of the American Mathematical Society},
    VOLUME = {72},
      YEAR = {1966},
     PAGES = {1--29},
      ISSN = {0002-9904},
   MRCLASS = {17.30 (16.90)},
  MRNUMBER = {195995},
MRREVIEWER = {G.\ Leger},
       DOI = {10.1090/S0002-9904-1966-11401-5},
       URL = {https://doi.org/10.1090/S0002-9904-1966-11401-5},
}

@article {MR0161898,
    AUTHOR = {Gerstenhaber, Murray},
     TITLE = {The cohomology structure of an associative ring},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {78},
      YEAR = {1963},
     PAGES = {267--288},
      ISSN = {0003-486X},
   MRCLASS = {16.90 (18.00)},
  MRNUMBER = {161898},
MRREVIEWER = {M.\ Auslander},
       DOI = {10.2307/1970343},
       URL = {https://doi.org/10.2307/1970343},
}

@article {MR0171807,
    AUTHOR = {Gerstenhaber, Murray},
     TITLE = {On the deformation of rings and algebras},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {79},
      YEAR = {1964},
     PAGES = {59--103},
      ISSN = {0003-486X},
   MRCLASS = {16.90 (13.93)},
  MRNUMBER = {171807},
MRREVIEWER = {D.\ Zelinsky},
       DOI = {10.2307/1970484},
       URL = {https://doi.org/10.2307/1970484},
}

@article {MR0083801,
    AUTHOR = {Fr\"{o}licher, Alfred and Nijenhuis, Albert},
     TITLE = {A theorem on stability of complex structures},
   JOURNAL = {Proc. Nat. Acad. Sci. U.S.A.},
  FJOURNAL = {Proceedings of the National Academy of Sciences of the United
              States of America},
    VOLUME = {43},
      YEAR = {1957},
     PAGES = {239--241},
      ISSN = {0027-8424},
   MRCLASS = {53.3X},
  MRNUMBER = {83801},
MRREVIEWER = {M.\ F.\ Atiyah},
       DOI = {10.1073/pnas.43.2.239},
       URL = {https://doi.org/10.1073/pnas.43.2.239},
}

@Article{zbMATH02694718,
 Author = {Noether, M.},
 Title = {Anzahl der {Moduln} einer {Klasse} algebraischer {Fl{\"a}chen}.},
 FJournal = {Sitzungsberichte der K{\"o}niglich Preussischen Akademie der Wissenschaften},
 Journal = {Berl. Ber.},
 Volume = {1888},
 Pages = {123--128},
 Year = {1888},
 Language = {German},
 zbMATH = {2694718},
 JFM = {20.0794.04}
}

@article {MR1579035,
    AUTHOR = {Riemann, B.},
     TITLE = {Theorie der {A}bel'schen {F}unctionen},
   JOURNAL = {J. Reine Angew. Math.},
  FJOURNAL = {Journal f\"{u}r die Reine und Angewandte Mathematik. [Crelle's
              Journal]},
    VOLUME = {54},
      YEAR = {1857},
     PAGES = {115--155},
      ISSN = {0075-4102,1435-5345},
   MRCLASS = {99-04},
  MRNUMBER = {1579035},
       DOI = {10.1515/crll.1857.54.115},
       URL = {https://doi.org/10.1515/crll.1857.54.115},
}

@article {DDT,
	AUTHOR = {Drinfeld, V.},
	TITLE = {A letter from {K}harkov to {M}oscow},
	NOTE = {Translated from the Russian by Keith Conrad},
	JOURNAL = {EMS Surv. Math. Sci.},
	FJOURNAL = {EMS Surveys in Mathematical Sciences},
	VOLUME = {1},
	YEAR = {2014},
	NUMBER = {2},
	PAGES = {241--248},
	ISSN = {2308-2151},
	MRCLASS = {18G55 (14D15 17B55)},
	MRNUMBER = {3285856},
	DOI = {10.4171/EMSS/5},
	URL = {https://doi.org/10.4171/EMSS/5},
}

@article {KodairaSpencer,
	AUTHOR = {Kodaira, K. and Spencer, D. C.},
	TITLE = {On deformations of complex analytic structures. {I}, {II}},
	JOURNAL = {Ann. of Math. (2)},
	FJOURNAL = {Annals of Mathematics. Second Series},
	VOLUME = {67},
	YEAR = {1958},
	PAGES = {328--466},
	ISSN = {0003-486X},
	MRCLASS = {57.00},
	MRNUMBER = {112154},
	MRREVIEWER = {M. F. Atiyah},
	DOI = {10.2307/1970009},
	URL = {https://doi.org/10.2307/1970009},
}

@article {toen_azumaya,
    AUTHOR = {To\"en, Bertrand},
     TITLE = {Derived {A}zumaya algebras and generators for twisted derived
              categories},
   JOURNAL = {Invent. Math.},
  FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {189},
      YEAR = {2012},
    NUMBER = {3},
     PAGES = {581--652},
      ISSN = {0020-9910,1432-1297},
   MRCLASS = {18E30 (14F05 14F20 16E35 18D10 18G55)},
  MRNUMBER = {2957304},
MRREVIEWER = {Julia\ Bergner},
       DOI = {10.1007/s00222-011-0372-1},
       URL = {https://doi.org/10.1007/s00222-011-0372-1},
}

@article {antieau_gepner_brauer_groups,
    AUTHOR = {Antieau, Benjamin and Gepner, David},
     TITLE = {Brauer groups and \'etale cohomology in derived algebraic
              geometry},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry \& Topology},
    VOLUME = {18},
      YEAR = {2014},
    NUMBER = {2},
     PAGES = {1149--1244},
      ISSN = {1465-3060,1364-0380},
   MRCLASS = {14F22 (13D09 14D20 18G55 55P43)},
  MRNUMBER = {3190610},
MRREVIEWER = {Timothy\ J.\ Ford},
       DOI = {10.2140/gt.2014.18.1149},
       URL = {https://doi.org/10.2140/gt.2014.18.1149},
}


@article {hinich,
	AUTHOR = {Hinich, Vladimir},
	TITLE = {Homological algebra of homotopy algebras},
	JOURNAL = {Comm. Algebra},
	FJOURNAL = {Communications in Algebra},
	VOLUME = {25},
	YEAR = {1997},
	NUMBER = {10},
	PAGES = {3291--3323},
	ISSN = {0092-7872},
	MRCLASS = {18G99 (16E99 18G05 55U35)},
	MRNUMBER = {1465117},
	MRREVIEWER = {Kathryn P. Hess},
	DOI = {10.1080/00927879708826055},
	URL = {https://doi.org/10.1080/00927879708826055},
}


@article {hinichcoalgebras,
	AUTHOR = {Hinich, Vladimir},
	TITLE = {D{G} coalgebras as formal stacks},
	JOURNAL = {J. Pure Appl. Algebra},
	FJOURNAL = {Journal of Pure and Applied Algebra},
	VOLUME = {162},
	YEAR = {2001},
	NUMBER = {2-3},
	PAGES = {209--250},
	ISSN = {0022-4049},
	MRCLASS = {14B12 (16W30 18G55 55P62)},
	MRNUMBER = {1843805},
	MRREVIEWER = {Paul G. Goerss},
	DOI = {10.1016/S0022-4049(00)00121-3},
	URL = {https://doi.org/10.1016/S0022-4049(00)00121-3},
}


@article {pridham,
	AUTHOR = {Pridham, J. P.},
	TITLE = {Unifying derived deformation theories},
	JOURNAL = {Adv. Math.},
	FJOURNAL = {Advances in Mathematics},
	VOLUME = {224},
	YEAR = {2010},
	NUMBER = {3},
	PAGES = {772--826},
	ISSN = {0001-8708},
	MRCLASS = {14B12 (16E35)},
	MRNUMBER = {2628795},
	MRREVIEWER = {Eivind Eriksen},
	DOI = {10.1016/j.aim.2009.12.009},
	URL = {https://doi.org/10.1016/j.aim.2009.12.009},
}


@article {dagsurvey,
	AUTHOR = {To\"{e}n, Bertrand},
	TITLE = {Derived algebraic geometry},
	JOURNAL = {EMS Surv. Math. Sci.},
	FJOURNAL = {EMS Surveys in Mathematical Sciences},
	VOLUME = {1},
	YEAR = {2014},
	NUMBER = {2},
	PAGES = {153--240},
	ISSN = {2308-2151},
	MRCLASS = {14A20 (14D15 18G55)},
	MRNUMBER = {3285853},
	MRREVIEWER = {Julia Bergner},
	DOI = {10.4171/EMSS/4},
	URL = {https://doi.org/10.4171/EMSS/4},
}


@book {complexcotangent1,
	AUTHOR = {Illusie, Luc},
	TITLE = {Complexe cotangent et d\'{e}formations. {I}},
	SERIES = {Lecture Notes in Mathematics, Vol. 239},
	PUBLISHER = {Springer-Verlag, Berlin-New York},
	YEAR = {1971},
	PAGES = {xv+355},
	MRCLASS = {14B10 (14D15 14F20 55D20)},
	MRNUMBER = {0491680},
	MRREVIEWER = {Larry Breen},
}


@misc{gammage2023perverse,
      title={Perverse schobers and 3d mirror symmetry}, 
      author={Benjamin Gammage and Justin Hilburn and Aaron Mazel-Gee},
      year={2023},
      eprint={2202.06833},
      archivePrefix={arXiv},
      primaryClass={math.RT}
}


@Book{fgaexplained,
title      = {Fundamental algebraic geometry},
publisher  = {American Mathematical Society, Providence, RI},
year       = {2005},
author     = {Fantechi, Barbara and G\"ottsche, Lothar and Illusie, Luc and Kleiman, Steven L. and Nitsure, Nitin and Vistoli, Angelo},
volume     = {123},
series     = {Mathematical Surveys and Monographs},
isbn       = {0-8218-3541-6},
note       = {Grothendieck's FGA explained},
mrclass    = {14-06 (14A15 14D15 14F20)},
mrnumber   = {2222646},
mrreviewer = {Liam O'Carroll},
pages      = {x+339},
}


@misc{CG,
	title={Formal moduli problems and formal derived stacks}, 
	author={Damien Calaque and Julien Grivaux},
	year={2019},
	eprint={1802.09556},
	archivePrefix={arXiv},
	primaryClass={math.AG}
}


@Book{fga,
title      = {Fondements de la g\'eom\'etrie alg\'ebrique. [{E}xtraits du {S}\'eminaire {B}ourbaki, 1957--1962.]},
publisher  = {Secr\'etariat math\'ematique, Paris},
year       = {1962},
author     = {Grothendieck, Alexander},
mrclass    = {14.00},
mrnumber   = {0146040},
mrreviewer = {E. L. Griffin, Jr.},
pages      = {ii+205},
}


@InCollection{descente,
author    = {Grothendieck, Alexander},
title     = {Technique de descente et th\'eor\`emes d'existence en g\'eometrie alg\'ebrique. {I}. {G}\'en\'eralit\'es. {D}escente par morphismes fid\`element plats},
booktitle = {S\'eminaire {B}ourbaki, {V}ol.\ 5},
publisher = {Soc. Math. France, Paris},
year      = {1995},
pages     = {Exp.\ No.\ 190, 299--327},
mrclass   = {14A15},
mrnumber  = {1603475},
}


@Book{hartshorne,
title      = {Algebraic geometry},
publisher  = {Springer-Verlag, New York-Heidelberg},
year       = {1977},
author     = {Hartshorne, Robin},
isbn       = {0-387-90244-9},
note       = {Graduate Texts in Mathematics, No. 52},
mrclass    = {14-01},
mrnumber   = {0463157},
mrreviewer = {Robert Speiser},
pages      = {xvi+496},
}


@Book{hodge,
title     = {The theory and applications of harmonic integrals},
publisher = {Cambridge University Press, Cambridge},
year      = {1989},
author    = {Hodge, W. V. D.},
series    = {Cambridge Mathematical Library},
isbn      = {0-521-35881-7},
note      = {Reprint of the 1941 original, With a foreword by Michael Atiyah},
mrclass   = {58A14 (01A60 01A75 32G20 53-02)},
mrnumber  = {1015714},
pages     = {xiv+284},
}


@Article{hironaka,
author     = {Hironaka, Heisuke},
title      = {Resolution of singularities of an algebraic variety over a field of characteristic zero. {I}, {II}},
journal    = {Ann. of Math. (2) {\bf 79} (1964), 109--203; ibid. (2)},
year       = {1964},
volume     = {79},
pages      = {205--326},
issn       = {0003-486X},
fjournal   = {Annals of Mathematics. Second Series},
mrclass    = {14.18},
mrnumber   = {0199184},
mrreviewer = {J. Giraud},
}


@Book{liu,
title      = {Algebraic geometry and arithmetic curves},
publisher  = {Oxford University Press, Oxford},
year       = {2002},
author     = {Liu, Qing},
volume     = {6},
series     = {Oxford Graduate Texts in Mathematics},
isbn       = {0-19-850284-2},
note       = {Translated from the French by Reinie Ern\'e, Oxford Science Publications},
mrclass    = {14-01 (11G30 14A05 14A15 14Gxx 14Hxx)},
mrnumber   = {1917232},
mrreviewer = {C\~A-cero Carvalho},
pages      = {xvi+576},
}


@Book{mazurmessing,
title      = {Universal extensions and one dimensional crystalline cohomology},
publisher  = {Springer-Verlag, Berlin-New York},
year       = {1974},
author     = {Mazur, B. and Messing, William},
series     = {Lecture Notes in Mathematics, Vol. 370},
mrclass    = {14K05 (14F30 14G05 14L05)},
mrnumber   = {0374150},
mrreviewer = {S. Bloch},
pages      = {vii+134},
}


@Book{mumford,
title      = {Geometric invariant theory},
publisher  = {Springer-Verlag, Berlin-New York},
year       = {1965},
author     = {Mumford, David},
series     = {Ergebnisse der Mathematik und ihrer Grenzgebiete, Neue Folge, Band 34},
mrclass    = {14.55},
mrnumber   = {0214602},
mrreviewer = {F. Oort},
pages      = {vi+145},
}


@Article{murre,
author     = {Murre, J. P.},
title      = {On contravariant functors from the category of pre-schemes over a field into the category of abelian groups (with an application to the {P}icard functor)},
journal    = {Inst. Hautes \'Etudes Sci. Publ. Math.},
year       = {1964},
number     = {23},
pages      = {5--43},
issn       = {0073-8301},
fjournal   = {Institut des Hautes \'Etudes Scientifiques. Publications Math\'ematiques},
mrclass    = {14.55},
mrnumber   = {0206011},
mrreviewer = {J. R. Isbell},
url        = {http://www.numdam.org/item?id=PMIHES_1964__23__5_0},
}


@Article{Oort,
author     = {Oort, F.},
title      = {Algebraic group schemes in characteristic zero are reduced},
journal    = {Invent. Math.},
year       = {1966},
volume     = {2},
pages      = {79--80},
issn       = {0020-9910},
doi        = {10.1007/BF01403391},
fjournal   = {Inventiones Mathematicae},
mrclass    = {14.50},
mrnumber   = {0206005},
mrreviewer = {S. S. Shatz},
url        = {http://dx.doi.org/10.1007/BF01403391},
}


@Book{oort2,
title         = {Commutative group schemes},
publisher     = {Springer-Verlag, Berlin-New York},
year          = {1966},
author        = {Oort, F.},
volume        = {15},
series        = {Lecture Notes in Mathematics},
__markedentry = {[Emanuele:1]},
mrclass       = {14.50 (18.00)},
mrnumber      = {0213365},
mrreviewer    = {S. S. Shatz},
pages         = {vi+133 pp. (not consecutively paged)},
}


@Book{steenbrink,
title      = {Mixed {H}odge structures},
publisher  = {Springer-Verlag, Berlin},
year       = {2008},
author     = {Peters, Chris A. M. and Steenbrink, Joseph H. M.},
volume     = {52},
series     = {Ergebnisse der Mathematik und ihrer Grenzgebiete. 3. Folge. A Series of Modern Surveys in Mathematics [Results in Mathematics and Related Areas. 3rd Series. A Series of Modern Surveys in Mathematics]},
isbn       = {978-3-540-77015-2},
mrclass    = {14C30 (14D07 32G20 32J25 32S35)},
mrnumber   = {2393625},
mrreviewer = {Matt Kerr},
pages      = {xiv+470},
}


@Book{raynaud,
title      = {Faisceaux amples sur les sch\'emas en groupes et les espaces homog\`enes},
publisher  = {Springer-Verlag, Berlin-New York},
year       = {1970},
author     = {Raynaud, Michel},
series     = {Lecture Notes in Mathematics, Vol. 119},
mrclass    = {14.55},
mrnumber   = {0260758},
mrreviewer = {D. Gieseker},
pages      = {ii+218},
}


@Article{gaga,
author     = {Serre, Jean-Pierre},
title      = {G\'eom\'etrie alg\'ebrique et g\'eom\'etrie analytique},
journal    = {Ann. Inst. Fourier, Grenoble},
year       = {1955--1956},
volume     = {6},
pages      = {1--42},
issn       = {0373-0956},
fjournal   = {Universit\'e de Grenoble. Annales de l'Institut Fourier},
mrclass    = {53.3X},
mrnumber   = {0082175},
mrreviewer = {H. Cartan},
url        = {http://aif.cedram.org/item?id=AIF_1955__6__1_0},
}


@Book{motives,
title      = {Cycles, transfers, and motivic homology theories},
publisher  = {Princeton University Press, Princeton, NJ},
year       = {2000},
author     = {Voevodsky, Vladimir and Suslin, Andrei and Friedlander, Eric M.},
volume     = {143},
series     = {Annals of Mathematics Studies},
isbn       = {0-691-04814-2; 0-691-04815-0},
mrclass    = {14F42 (14C25 19E15)},
mrnumber   = {1764197},
mrreviewer = {Spencer J. Bloch},
pages      = {vi+254},
}


@Book{sga3,
title     = {S\'eminaire de G\'eom\'etrie Alg\'ebrique du Bois-Marie},
publisher = {Springer-Verlag},
year      = {1970-1973},
author    = {Grothendieck, Alexander and Raynaud, Mich\`ele and Demazure, Michel and Artin, Michael and Verdier, Jean-Louis and Deligne, Pierre and Berthelot, Pierre and Illusie, Luc and Katz, Nicholas},
address   = {Berlin},
note      = {Lecture Notes in Mathematics, Vols. 151, 152, 153, 224, 225, 269, 270, 288, 305, 340, 569, and 589},
}


@Book{ega,
title     = {\'{E}l\'ements de g\'eom\'etrie alg\'ebrique.},
publisher = {Inst. Hautes \'Etudes Sci. Publ. Math.},
year      = {1960-1967},
author    = {Grothendieck, Alexander and Dieudonn\'e, Jean-Alexandre-Eug\`ene},
number    = {4, 8, 11, 17, 20, 24, 28, and 32},
note      = {Institut des Hautes \'Etudes Scientifiques. Publications Math\'ematiques},
fjournal  = {Institut des Hautes \'Etudes Scientifiques. Publications Math\'ematiques},
issn      = {0073-8301},
mrclass   = {14.55},
}


@Misc{milne2,
author       = {Milne, James S.},
title        = {Algebraic Groups},
howpublished = {http://www.jmilne.org/math/CourseNotes/iAG200.pdf},
month        = {Dec},
year         = {2015},
}


@Misc{pink,
author       = {Pink, Richard},
title        = {Finite group schemes},
howpublished = {https://people.math.ethz.ch/~pink/ftp/FGS/CompleteNotes.pdf},
year         = {2004/2005},
note         = {Lecture notes.},
}


@Article{andre,
author  = {Yves Andr\`e},
title   = {Une introduction aux motifs (motifs purs, motifs mixtes, p\`eriodes)},
journal = {Panoramas et Synth\'eses [Panoramas and Syntheses], vol. 17},
year    = {2004},
}


@Article{tabuada,
author  = {Gonçalo Tabuada},
title   = {Noncommutative Motives},
journal = {American Mathematical Society University Lecture Series},
year    = {2010},
volume  = {63},
}


@Misc{voevconjecture,
author       = {Marcello Bernardara, and Matilde Marcolli, and Gonçalo Tabuada},
title        = {Some remarks concerning Voevodsky’s nilpotence conjecture},
howpublished = {https://arxiv.org/pdf/0912.2110.pdf},
journal      = {arXiv:1403.0876(v3).},
}


@Article{kahnsebastian,
author  = {Bruno Kahn and Ronnie Sebastian},
title   = {Smash-nilpotent cycles on abelian 3-folds},
journal = {Math. Res. Lett. 16},
year    = {2009},
volume  = {6},
pages   = {1007–1010},
}


@Article{matsusaka,
author  = {Teruhisa Matsusaka},
title   = {The criteria for algebraic equivalence and the torsion group},
journal = {Amer. J. Math. 79},
year    = {1957},
pages   = {53-66},
}


@Article{voevodskynilpotence,
author  = {Vladimir Voevodsky},
title   = {A nilpotence theorem for cycles algebraically equivalent to zero},
journal = {Internat. Math. Res. Notices},
year    = {1995},
volume  = {4},
pages   = {187-198},
}


@article {joyce,
AUTHOR = {Brav, Christopher and Bussi, Vittoria and Joyce, Dominic},
TITLE = {A {D}arboux theorem for derived schemes with shifted
	symplectic structure},
JOURNAL = {J. Amer. Math. Soc.},
FJOURNAL = {Journal of the American Mathematical Society},
VOLUME = {32},
YEAR = {2019},
NUMBER = {2},
PAGES = {399--443},
ISSN = {0894-0347},
MRCLASS = {14A20 (14D23 14F05 14N35)},
MRNUMBER = {3904157},
MRREVIEWER = {Hsian-Hua Tseng},
DOI = {10.1090/jams/910},
URL = {https://doi.org/10.1090/jams/910},
}


@book{chriss2009representation,
  title={Representation Theory and Complex Geometry},
  author={Chriss, N. and Ginzburg, V.},
  isbn={9780817649388},
  lccn={94027574},
  series={Modern Birkh{\"a}user Classics},
  url={https://books.google.it/books?id=OZlCAAAAQBAJ},
  year={2009},
  publisher={Birkh{\"a}user Boston}
}




@Misc{rozenblyum2018talk,
AUTHOR = {Rozenblyum, Nick},
TITLE = {Topological Chiral Categories},
YEAR = {2018},
NOTE = {Winter school on local geometric Langlands theory},
URL = {https://lysenko.perso.math.cnrs.fr/Notes_talks_winter2018/T-5(Nick).pdf},
}


@misc{hedenlund2023twisted,
      title={Twisted Spectra Revisited}, 
      author={Alice Hedenlund and Tasos Moulinos},
      year={2023},
      eprint={2312.07403},
      archivePrefix={arXiv},
      primaryClass={math.AT}
}


@incollection {hopfgalois,
	AUTHOR = {Hess, Kathryn},
	TITLE = {Homotopic {H}opf-{G}alois extensions: foundations and
		examples},
	BOOKTITLE = {New topological contexts for {G}alois theory and algebraic
		geometry ({BIRS} 2008)},
	SERIES = {Geom. Topol. Monogr.},
	VOLUME = {16},
	PAGES = {79--132},
	PUBLISHER = {Geom. Topol. Publ., Coventry},
	YEAR = {2009},
	MRCLASS = {55P42 (16T05 18D10 55U35 57T30)},
	MRNUMBER = {2544387},
	MRREVIEWER = {John Hunton},
	DOI = {10.2140/gtm.2009.16.79},
	URL = {https://doi.org/10.2140/gtm.2009.16.79},
}


@article {hinichyoneda,
	AUTHOR = {Hinich, Vladimir},
	TITLE = {Yoneda lemma for enriched {$\infty$}-categories},
	JOURNAL = {Adv. Math.},
	FJOURNAL = {Advances in Mathematics},
	VOLUME = {367},
	YEAR = {2020},
	PAGES = {107129, 119},
	ISSN = {0001-8708,1090-2082},
	MRCLASS = {18D20 (18M05)},
	MRNUMBER = {4080581},
	MRREVIEWER = {Luciano\ Stramaccia},
	DOI = {10.1016/j.aim.2020.107129},
	URL = {https://doi.org/10.1016/j.aim.2020.107129},
}


@article {dgcoalgebrasformalstacks,
	AUTHOR = {Hinich, Vladimir},
	TITLE = {D{G} coalgebras as formal stacks},
	JOURNAL = {J. Pure Appl. Algebra},
	FJOURNAL = {Journal of Pure and Applied Algebra},
	VOLUME = {162},
	YEAR = {2001},
	NUMBER = {2-3},
	PAGES = {209--250},
	ISSN = {0022-4049},
	MRCLASS = {14B12 (16W30 18G55 55P62)},
	MRNUMBER = {1843805},
	MRREVIEWER = {Paul G. Goerss},
	DOI = {10.1016/S0022-4049(00)00121-3},
	URL = {https://doi.org/10.1016/S0022-4049(00)00121-3},
}


@book {weilhodge,
AUTHOR = {Weil, Andr\'{e}},
TITLE = {Introduction \`a l'\'{e}tude des vari\'{e}t\'{e}s k\"{a}hl\'{e}riennes},
SERIES = {Publications de l'Institut de Math\'{e}matique de l'Universit\'{e} de
	Nancago, VI. Actualit\'{e}s Sci. Ind. no. 1267},
PUBLISHER = {Hermann, Paris},
YEAR = {1958},
PAGES = {175},
MRCLASS = {57.00},
MRNUMBER = {0111056},
MRREVIEWER = {F. Hirzebruch},
}


@article {stanculescu,
	AUTHOR = {Stanculescu, Alexandru E.},
	TITLE = {A {Q}uillen model category structure on some categories of
		comonoids},
	JOURNAL = {J. Pure Appl. Algebra},
	FJOURNAL = {Journal of Pure and Applied Algebra},
	VOLUME = {214},
	YEAR = {2010},
	NUMBER = {5},
	PAGES = {629--633},
	ISSN = {0022-4049},
	MRCLASS = {55U35},
	MRNUMBER = {2577669},
	DOI = {10.1016/j.jpaa.2009.07.002},
	URL = {https://doi.org/10.1016/j.jpaa.2009.07.002},
}


@book {hirschhorn,
	AUTHOR = {Hirschhorn, Philip S.},
	TITLE = {Model categories and their localizations},
	SERIES = {Mathematical Surveys and Monographs},
	VOLUME = {99},
	PUBLISHER = {American Mathematical Society, Providence, RI},
	YEAR = {2003},
	PAGES = {xvi+457},
	ISBN = {0-8218-3279-4},
	MRCLASS = {18G55 (55P60 55U35)},
	MRNUMBER = {1944041},
	MRREVIEWER = {David A. Blanc},
	DOI = {10.1090/surv/099},
	URL = {https://doi.org/10.1090/surv/099},
}


@Article{voisin,
author  = {Claire Voisin},
title   = {Remarks on zero-cycles of self-products of varieties, Moduli of vector bundles},
journal = {Lecture Notes in Pure and Appl. Math.},
year    = {1994},
volume  = {179},
pages   = {265-285},
}


@Article{poonen,
author  = {Bjorn Poonen},
title   = {The Grothendieck ring of varieties is not a domain},
journal = {Math. Res. Lett. 9},
year    = {2002},
volume  = {4},
pages   = {493-497},
}


@Article{bll,
author  = {Alexey I. Bondal, and Michael Larsen, and Valery A. Lunts},
title   = {Grothendieck ring of pretriangulated categories},
journal = {Int. Math. Res. Not.},
year    = {2004},
volume  = {29},
pages   = {1461–1495},
}


@Misc{kuznetsov,
author       = {Alexander Kuznetsov},
title        = {Derived Categories of Quadric Fibrations and Intersections of Quadrics},
howpublished = {arXiv:math/0510670},
month        = oct,
year         = {2005},
}

@misc{savage2024representabilitytheoremstacksderived,
      title={A Representability Theorem for Stacks in Derived Geometry Contexts}, 
      author={Rhiannon Savage},
      year={2024},
      eprint={2405.08361},
      archivePrefix={arXiv},
      primaryClass={math.AG},
      url={https://arxiv.org/abs/2405.08361}, 
}


@book {mcduff-salamon,
    AUTHOR = {McDuff, Dusa and Salamon, Dietmar},
     TITLE = {Introduction to symplectic topology},
    SERIES = {Oxford Mathematical Monographs},
   EDITION = {Second},
 PUBLISHER = {The Clarendon Press, Oxford University Press, New York},
      YEAR = {1998},
     PAGES = {x+486},
      ISBN = {0-19-850451-9},
   MRCLASS = {53D35 (53D40 57R17 57R57 57R58)},
  MRNUMBER = {1698616},
MRREVIEWER = {Hansj\"org\ Geiges},
}


@article {savelyev,
    AUTHOR = {Savelyev, Yasha},
     TITLE = {Global {F}ukaya category {I}},
   JOURNAL = {Int. Math. Res. Not. IMRN},
  FJOURNAL = {International Mathematics Research Notices. IMRN},
      YEAR = {2023},
    NUMBER = {21},
     PAGES = {18302--18386},
      ISSN = {1073-7928,1687-0247},
   MRCLASS = {14F08 (18G70 18N20 53D05 53D37)},
  MRNUMBER = {4665626},
       DOI = {10.1093/imrn/rnad013},
       URL = {https://doi.org/10.1093/imrn/rnad013},
}


@article {oh-tanaka,
    AUTHOR = {Oh, Yong-Geun and Tanaka, Hiro Lee},
     TITLE = {Smooth constructions of homotopy-coherent actions},
   JOURNAL = {Algebr. Geom. Topol.},
  FJOURNAL = {Algebraic \& Geometric Topology},
    VOLUME = {22},
      YEAR = {2022},
    NUMBER = {3},
     PAGES = {1177--1216},
      ISSN = {1472-2747,1472-2739},
   MRCLASS = {58B05 (53D37 58D05)},
  MRNUMBER = {4474782},
       DOI = {10.2140/agt.2022.22.1177},
       URL = {https://doi.org/10.2140/agt.2022.22.1177},
}

@article {serre_homotopy_groups,
    AUTHOR = {Serre, Jean-Pierre},
     TITLE = {Groupes d'homotopie et classes de groupes ab\'eliens},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {58},
      YEAR = {1953},
     PAGES = {258--294},
      ISSN = {0003-486X},
   MRCLASS = {56.0X},
  MRNUMBER = {59548},
MRREVIEWER = {W.\ S.\ Massey},
       DOI = {10.2307/1969789},
       URL = {https://doi.org/10.2307/1969789},
}

@book {May_Ponto,
    AUTHOR = {May, J. P. and Ponto, K.},
     TITLE = {More concise algebraic topology},
    SERIES = {Chicago Lectures in Mathematics},
      NOTE = {Localization, completion, and model categories},
 PUBLISHER = {University of Chicago Press, Chicago, IL},
      YEAR = {2012},
     PAGES = {xxviii+514},
      ISBN = {978-0-226-51178-8; 0-226-51178-2},
   MRCLASS = {55-02 (16T05 18G55 55P60)},
  MRNUMBER = {2884233},
MRREVIEWER = {Ismar\ Voli\'c},
}

@book {FHTrational,
    AUTHOR = {F\'elix, Yves and Halperin, Stephen and Thomas, Jean-Claude},
     TITLE = {Rational homotopy theory},
    SERIES = {Graduate Texts in Mathematics},
    VOLUME = {205},
 PUBLISHER = {Springer-Verlag, New York},
      YEAR = {2001},
     PAGES = {xxxiv+535},
      ISBN = {0-387-95068-0},
   MRCLASS = {55P62 (18Gxx 55U35)},
  MRNUMBER = {1802847},
MRREVIEWER = {John\ F.\ Oprea},
       DOI = {10.1007/978-1-4613-0105-9},
       URL = {https://doi.org/10.1007/978-1-4613-0105-9},
}

@article {Vigue-Poirrier_Sullivan,
    AUTHOR = {Vigu\'e-Poirrier, Micheline and Sullivan, Dennis},
     TITLE = {The homology theory of the closed geodesic problem},
   JOURNAL = {J. Differential Geometry},
  FJOURNAL = {Journal of Differential Geometry},
    VOLUME = {11},
      YEAR = {1976},
    NUMBER = {4},
     PAGES = {633--644},
      ISSN = {0022-040X,1945-743X},
   MRCLASS = {58E10},
  MRNUMBER = {455028},
MRREVIEWER = {Peter\ Klein},
       URL = {http://projecteuclid.org/euclid.jdg/1214433729},
}

@incollection {Hess_Rational,
    AUTHOR = {Hess, Kathryn},
     TITLE = {Rational homotopy theory: a brief introduction},
 BOOKTITLE = {Interactions between homotopy theory and algebra},
    SERIES = {Contemp. Math.},
    VOLUME = {436},
     PAGES = {175--202},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2007},
      ISBN = {978-0-8218-3814-3},
   MRCLASS = {55P62 (55M30)},
  MRNUMBER = {2355774},
MRREVIEWER = {Yves\ F\'elix},
       DOI = {10.1090/conm/436/08409},
       URL = {https://doi.org/10.1090/conm/436/08409},
}

@article {ayala-francis,
    AUTHOR = {Ayala, David and Francis, John},
     TITLE = {Factorization homology of topological manifolds},
   JOURNAL = {J. Topol.},
  FJOURNAL = {Journal of Topology},
    VOLUME = {8},
      YEAR = {2015},
    NUMBER = {4},
     PAGES = {1045--1084},
      ISSN = {1753-8416,1753-8424},
   MRCLASS = {55U40 (57N35 57R19 57R56)},
  MRNUMBER = {3431668},
MRREVIEWER = {Jason\ Stuart\ Hanson},
       DOI = {10.1112/jtopol/jtv028},
       URL = {https://doi.org/10.1112/jtopol/jtv028},
}


@Comment{jabref-meta: databaseType:bibtex;}

